Look Carefully: Adaptive Visual Reinforcements in Multimodal Large Language Models for Hallucination Mitigation

Multimodal large language models (MLLMs) have achieved remarkable progress in vision-language reasoning, yet they remain vulnerable to hallucination, where generated content deviates from visual evidence. Existing mitigation strategies either require costly supervision during training or introduce additional latency at inference time. Recent vision enhancement methods attempt to address this issue by reinforcing visual tokens during decoding, but they typically inject all tokens indiscriminately, which causes interference from background regions and distracts the model from critical cues. To overcome this challenge, we propose Adaptive Visual Reinforcement (AIR), a training-free framework for MLLMs. AIR consists of two components. Prototype-based token reduction condenses the large pool of visual tokens into a compact subset to suppress redundancy. OT-guided patch reinforcement quantifies the alignment between hidden states and patch embeddings to selectively integrate the most consistent patches into feed-forward layers. As a result, AIR enhances the model's reliance on salient visual information and effectively mitigates hallucination. Extensive experiments across representative MLLMs demonstrate that AIR substantially reduces hallucination while preserving general capabilities, establishing it as an effective solution for building reliable MLLMs.

==> 2026_ICLR/figures/case.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{2026_ICLR/figures/case_study.pdf}
    % \vspace{-15pt}
    \caption{\textbf{.}.
    }
    % \label{Fig_motivation}
\end{figure}


==> 2026_ICLR/sections/3_method.tex <==
\section{Method}
\subsection{Preliminaries}\label{sec:prelims}
\textbf{\noindent{Multi-modal large language models.}} 
Multi-modal Large Language Models (MLLMs) extend conventional LLMs to jointly process text and images. An MLLM typically consists of a vision encoder $\Phi$, a vision--language interface $G$, and an autoregressive text decoder. Given a textual query $x=\{x_1,\dots,x_L\}$ and an image $v$, the vision encoder extracts visual features $\V=\Phi(v)$, which are then mapped by the projector $G$~\citep{projector, projector1} into aligned visual tokens $\mathbf{Z}=G(\mathbf{V})=[\z_1, \z_2, \cdots, \z_K]$. 
Let $\{\mathbf{x}_1,\dots,\mathbf{x}_L\}$ denote the embeddings of $x$ produced by the text embedding layer, and define the multimodal input sequence
\begin{equation}
    \mathbf{X} = [\,\mathbf{Z}_v,\; \mathbf{x}_1,\dots,\mathbf{x}_L\,].
\end{equation}
At decoding step $t$, the transformer-based decoder produces unnormalized logits $f_\theta(\cdot \mid \mathbf{X}, y_{<t})$, from which the next-token distribution is obtained via the softmax:
\begin{equation}
    p_\theta(\cdot \mid \mathbf{X}, y_{<t})=\mathrm{softmax}\!\big(f_\theta(\cdot \mid \mathbf{X}, y_{<t})\big), 
    \qquad
    y_t \sim p_\theta(\cdot \mid \mathbf{X}, y_{<t}), \;\; t=1,\dots,T.
\end{equation}
Here, $\theta$ denotes all model parameters and $y_{<t}$ is the previously generated tokens. 



\textbf{\noindent{Optimal transport.}}
Optimal Transport (OT)~\citep{monge1781memoire} offers a principled framework for quantifying the discrepancy between two probability distributions. 
Consider two discrete measures in the feature space:
$\mathbb{P} = \sum_{i=1}^{|V|} a_i \delta_{\mathbf{v}_i}$ and $\mathbb{Q} = \sum_{j=1}^{|U|} b_j \delta_{\mathbf{u}_j}$,
where $\delta$ denotes the Dirac delta function, and $|V|$ and $|U|$ are the number of support points in $\mathbb{P}$ and $\mathbb{Q}$, respectively.
Here, $\mathbf{a} = [a_1,\dots,a_{|V|}]^\top$ and $\mathbf{b} = [b_1,\dots,b_{|U|}]^\top$ are probability vectors that sum to one. 
Given a cost matrix $\mathbf{C} \in \mathbb{R}^{|V|\times|U|}$, where $\mathbf{C}(i, j)$ is the element in $\mathbf{C}$, denoting the cost of transporting unit mass from $\mathbf{v}_i$ to $\mathbf{u}_j$, and the OT distance between $\mathbb{P}$ and $\mathbb{Q}$ is formulated as:
\begin{equation}
\label{eq:optimization}
d_{\mathrm{OT}}(\mathbb{P},\mathbb{Q};\mathbf{C}) = 
\min_{\mathbf{T}} \langle \mathbf{T}, \mathbf{C} \rangle, 
\quad
\text{s.t. } \mathbf{T}\mathbbm{1}_{|U|} = \mathbf{a}, \;\;  \mathbf{T}^\top \mathbbm{1}_{|V|} = \mathbf{b},
\end{equation}
where $\mathbf{T} \in \mathbb{R}^{|V|\times|U|}$ is the transport plan specifying how mass is moved between the two distributions. 
The notation $\langle \cdot,\cdot \rangle$ denotes the Frobenius inner product, and $\mathbbm{1}_{|V|}$ is an all-ones vector of dimension $|V|$. Directly solving Eq.~\eqref{eq:optimization} is computationally intensive. 
Prior work~\citep{iLPC, chen2023plot} addresses this by employing the Sinkhorn algorithm~\citep{cuturi2013sinkhorn}, which introduces entropic regularization to achieve efficient optimization:
\begin{equation}
\label{eq:opt_Sink}
d_{\mathrm{OT}}(\mathbb{P}, \mathbb{Q};\mathbf{C}) = 
\min_{\mathbf{T}} \langle \mathbf{T}, \mathbf{C} \rangle - \epsilon h(\mathbf{T}),
\end{equation}
where $h(\cdot)$ denotes the entropy and $\epsilon \geq 0$ controls the strength of the regularization.

\input{2026_ICLR/figures/framework}


\subsection{SELECTIVE VISUAL REINFORCEMENT}

\noindent{\textbf{Prototype-based Visual Token Selection.}}
The visual tokens $\mathbf{H}_v=[\mathbf{h}_1,\dots,\mathbf{h}_K]$ extracted in the hidden states carry rich semantic details. However, their number can be very large (e.g., $K=576$ in LLaVA), which not only introduces redundancy but also increases computational burden in subsequent layers. Empirically, many of these tokens correspond to visually similar or background regions and contribute little to semantic grounding. To alleviate redundancy while preserving critical information, we propose a prototype-based selection mechanism that condenses $\mathbf{H}_v$ into a more compact and informative subset.  

We first compute a global prototype vector $\mathbf{h}_{\mathrm{p}}$ as the mean of all visual tokens:
\begin{equation}
    \mathbf{h}_{\mathrm{p}} = \frac{1}{K}\sum_{k=1}^{K} \mathbf{h}_k.
\end{equation}
This prototype provides a coarse summary of the overall visual semantics and acts as a reference point for identifying distinctive tokens. Intuitively, tokens that deviate more from this prototype encode unique visual cues (e.g., salient objects or attributes) that are underrepresented by the global average.  

For each visual token, we compute its deviation from the prototype using the $\ell_2$ distance:
\begin{equation}
    d(\mathbf{h}_k,\mathbf{h}_{\mathrm{p}}) = \|\mathbf{h}_k - \mathbf{h}_{\mathrm{p}}\|_2,
    \qquad k=1,\dots,K.
\end{equation}
Larger distances indicate tokens with higher uniqueness and thus potentially greater contribution to visual grounding. Unlike uniform token retention, this distance-based measure prioritizes tokens that capture salient, non-redundant details.  

Based on the distance scores $\{d(\mathbf{h}_k,\mathbf{h}_{\mathrm{p}})\}_{k=1}^K$, we select the top-$k$ most distinctive tokens:
\begin{equation}
    \mathcal{V} = \operatorname{Top}\text{-}k\!\left(\{d(\mathbf{h}_k,\mathbf{h}_{\mathrm{p}})\}\right),
    \qquad
    \mathbf{H}_v \;\leftarrow\; \{\mathbf{h}_k \mid k \in \mathcal{V}\}.
\end{equation}
This reduces the token count from $K$ to $k$ ($k \ll K$), lowering computational cost while ensuring that the retained tokens are semantically diverse and informative. In this way, the subsequent reinforcement stage (Sec.~\ref{sec:analysis}) operates on a compact representation that emphasizes salient visual cues and avoids redundancy, thereby improving both efficiency and robustness.


\noindent{\textbf{Visual Reinforcement}}
% Following the attention calibration described in Section~\ref{sec:attention}, 在这个section, 我们介绍通过select critical的image patch来增强模型对视觉信息的利用，减弱幻觉的产生。具体来说
% the feed-forward network (FFN) in a Transformer block consists of two fully connected layers with a non-linear activation:
% Following the attention calibration described in Section~\ref{sec:attention}, 
% this section introduces a selective visual reinforcement approach that leverages critical image patches to enhance the utilization of visual information and mitigate hallucinations. 
% Specifically, the feed-forward network (FFN) in a Transformer block consists of two fully connected layers with a non-linear activation:
Following the attention calibration described in Section~\ref{sec:attention}, 
we propose a selective visual reinforcement strategy that focuses on critical image patches to reinforce visual cues and reduce hallucinations. 
Our selective visual reinforcement is performed in the feed-forward network (FFN) of each Transformer block, 
which consists of two fully connected layers with a non-linear activation:
\begin{equation}
    \mathrm{FFN}(\mathbf{H})
    = \phi\!\left(\mathbf{H}\,\mathbf{W}_1\right)\,\mathbf{W}_2^{\top},
\end{equation}
where $\phi(\cdot)$ denotes the activation function and $\mathbf{H}$ represents the hidden states. 
As the Transformer goes deeper, attention tends to become progressively biased towards textual tokens, 
which diminishes the contribution of visual tokens in later layers. 
To mitigate this imbalance, a common approach is to re-inject visual tokens into the FFN:
\begin{equation}
  \hat{\mathbf{W}}_1^{\top}
  = \mathbf{W}_1^{\top}
    + \cos_F(\mathbf{Z},\mathbf{W}_1^{\top})\,\mathbf{Z},
  \qquad
  \hat{\mathbf{W}}_2
  = \mathbf{W}_2
    + \cos_F(\mathbf{\Z}^{\top},\mathbf{W}_2)\,\mathbf{V}^{\top},
\end{equation}
where $\mathbf{Z}$ denotes the visual tokens introduced in Sec.~\ref{sec:prelims}, 
and $\cos_F(\mathbf{A},\mathbf{B}) = \frac{\langle \mathbf{A},\mathbf{B}\rangle_F}{\|\mathbf{A}\|_F\,\|\mathbf{B}\|_F}$ is the Frobenius cosine similarity used as a scaling factor to preserve magnitude consistency. 
However, directly injecting the entire set of visual tokens may introduce redundancy and noise. 
To reinforce visual information while avoiding redundancy, 
we design a patch-level selection mechanism that emphasizes only the most critical cues.
Specifically, the input image is cropped into multiple patches $\{\hat{v}^m\}_{m=1}^M$, 
with corresponding embeddings $\{\hat{\mathbf{Z}}^m\}_{m=1}^{M}$, 
where each $\hat{\mathbf{Z}}^m = [\mathbf{z}^m_1, \mathbf{z}^m_2, \cdots, \mathbf{z}^m_N]$ encodes fine-grained visual details. 
We model the original image tokens and patch-level tokens as discrete distributions:
\begin{equation}
    \mathbb{P}(\z) = \sum_{k=1}^{K} a_k \delta(\mathbf{z}_k-\z), \quad 
    \mathbb{Q}_m(\hat{\z}) = \sum_{n=1}^{N} b^m_n \delta(\hat{\mathbf{z}}_n^m-\hat{\z}),
\end{equation}
where $\delta(\cdot)$ denotes the Dirac delta function, and $a_k$, $b_n^m$ are normalized importance weights. 
The alignment between $\mathbb{P}$ and $\mathbb{Q}_m$ is quantified using the OT distance:
\begin{equation}
    d_{\mathrm{OT}}(\mathbb{P}, \mathbb{Q}_m; \mathbf{C}_m) 
    = \min_{\mathbf{T}_m \ge 0} \langle \mathbf{T}_m, \mathbf{C}_m \rangle, 
    \quad \text{s.t.} \quad \mathbf{T}_m \mathbf{1}_K = \mathbf{a}, \; 
    \mathbf{T}_m^\top \mathbf{1}_N = \mathbf{b}_m,
\end{equation}
where $\mathbf{a}=[\tfrac{1}{K},\dots,\tfrac{1}{K}]^\top$, 
$\mathbf{b}_m=[\tfrac{1}{N},\dots,\tfrac{1}{N}]^\top$, 
and $\mathbf{C}_m(k,n)=1-\cos(\mathbf{z}_k,\hat{\mathbf{z}}_n^m)$. 
The transport plan $\mathbf{T}_m$ is efficiently obtained via the Sinkhorn-Knopp algorithm~\citepp{sinkhorn}. 
For each patch $m$, we compute an aggregated OT distance:
\begin{equation}
    d_{\mathrm{OT}}(m) = \sum_{k=1}^{K}\sum_{n=1}^{N}\mathbf{T}_m(k,n)\,\mathbf{C}_m(k,n). \label{eq:dotm}
\end{equation}
A lower OT distance indicates stronger alignment with the original image and thus suggests that the patch retains more critical visual information. 
We therefore select patches with threshodling $\tau$:
\begin{equation}
    \mathcal{M} = \{\, m \mid d_{\mathrm{OT}}(m) \le \tau \,\}.
\end{equation}
The embeddings of these selected patches are then fused with the original image tokens:
\begin{equation}
    \mathbf{Z} \;\leftarrow\; \operatorname{concat}\!\big(\mathbf{Z},\, \{\hat{\mathbf{Z}}^{\,m} \mid m \in \mathcal{M}\}\big).
\end{equation}
This selective fusion enriches the representation with critical image details, 
effectively reinforcing visual information in the model’s hidden states 

\subsection{Theoretical Analysis}\label{sec:analysis}
To validate the effectiveness of our OT-based patch selection in Dynamic Token Infusion, we compare the sensitivity of our OT distance metric $d_{\mathrm{OT}}(m)$ with the baseline cosine distance $d_{\cos}(m) = \frac{1}{KN} \sum_{k=1}^K \sum_{n=1}^N \C_m(k,n)$. In our framework, a patch $ m $ is selected as useful if $ d_{\mathrm{OT}}(m) \leq \tau $, as lower OT distances indicate stronger alignment with critical visual semantics. Conversely, for the cosine baseline, a patch is selected if $ d_{\cos}(m) \leq \tau_{\cos} $, reflecting lower average misalignment. We prove that the OT-based method achieves strictly higher sensitivity in distinguishing patches:
\begin{equation}\label{eq:ot_margin}
|d_{\mathrm{OT}}(m_1) - d_{\mathrm{OT}}(m_2)| > |d_{\cos}(m_1) - d_{\cos}(m_2)|,
\end{equation}
except in the degenerate case where $\C_{m_1} = \C_{m_2}$.

\paragraph{Why OT enhances patch selection sensitivity.}
The OT-based metric employs an adaptive transport plan $ \T_m $hel, computed via Sinkhorn-Knopp, which prioritizes low-cost alignments (high cosine similarities) between original and patch tokens. This adaptive weighting amplifies differences in semantic alignment, resulting in a larger separation $ |d_{\mathrm{OT}}(m_1) - d_{\mathrm{OT}}(m_2)| $ compared to the uniform weighting of $ d_{\cos} $, which averages all pairwise costs and dilutes discriminative features. The increased sensitivity ensures more precise identification of patches in $ \mathcal{M} $ that capture critical visual information, enhancing the robustness of token infusion (Section~\ref{sec:prelims}). A detailed proof is provided in Appendix~\ref{app:proof}.



% \subsection{Adaptive Attention Calibration}\label{sec:attention}
% Consider a decoder-only multimodal transformer with $L$ layers and $n_H$ heads per layer. In the $l$-th block, the self-attention of head $h$ is formulated as:
% \begin{equation}
% \mathbf{A}_{l,h} = \frac{\mathbf{Q}_{l,h}\mathbf{K}_{l,h}^{\top}}{\sqrt{d_k}},
% \qquad
% \mathbf{O}_{l,h} = \softmax(\mathbf{A}_{l,h})\,\mathbf{V}_{l,h},
% \label{eq:vanilla-attn}
% \end{equation}
% where $\mathbf{Q}_{l,h}, \mathbf{K}_{l,h}, \mathbf{V}_{l,h}\in\mathbb{R}^{n\times d_k}$ are the query, key and value matrices, with $n$ denoting the sequence length and $d_k$ is the hidden dimension. The attention matrix $\mathbf{A}_{l,h}\in\mathbb{R}^{n\times n}$ captures pairwise token similarities. A straightforward approach to strengthen attention toward image tokens is to multiply their corresponding logits:
% \begin{equation}
% \hat{\mathbf{A}}_{l,h} = \mathbf{A}_{l,h} + \alpha \,\mathbf{M}^{\mathrm{enh}}_{l,h}\!\circ \mathbf{A}_{l,h},
% \qquad
% \mathbf{M}^{\mathrm{enh}}_{l,h}(i,j)=\mathbb{I}(i\in\mathcal{T}, j\in\mathcal{V}),
% \label{eq:mul-enh}
% \end{equation}
% where $\alpha>1$ is the strengthening coefficient, $\mathcal{T}$ and $\mathcal{V}$ denote the index sets of text and image tokens, and $\circ$ is the Hadamard product. 
% Here $\mathbf{M}^{\mathrm{enh}}_{l,h}$ is a binary indicator mask, taking the value $1$ when $(i,j)$ matches the specified condition and $0$ otherwise. However, this naive scaling is sign-dependent: positive logits are enlarged, while negative logits are pushed further negative, thereby reducing their probability mass after softmax. This contradicts the intended goal of uniformly amplifying visual attention.
% To ensure monotonic amplification regardless of the original logit signs, we reformulate multiplicative rescaling in probability space as additive shifts in logit space. In addition to amplifying image tokens, we also apply mild suppression to system tokens, since their logits are typically dominant and can overshadow visual information during decoding. The shifts are parameterized as logarithms of two hyperparameters:
% \begin{equation}
% \hat{\alpha} \;=\; \ln(\alpha) \;>\; 0,
% \qquad
% \hat{\beta} \;=\; \ln(\beta) \;<\; 0,
% \label{eq:beta-alpha}
% \end{equation}
% where $\beta\in(0,1)$ providing suppression for system tokens. Based on these parameters, the shifted logits are defined as:
% \begin{equation}
% \tilde{\mathbf{A}}_{l,h}(i,j) \;=\;
% \begin{cases}
% \mathbf{A}_{l,h}(i,j) + \hat{\alpha} \,\mathbf{M}^{\mathrm{enh}}_{l,h}(i, j), & i\in\mathcal{T}, j\in\mathcal{V},\\[2pt]
% \mathbf{A}_{l,h}(i,j) + \hat{\beta} \,\mathbf{M}^{\mathrm{sup}}_{l,h}(i, j), & i\in\mathcal{T}, j\in\mathcal{S}.
% \end{cases}
% \label{eq:shifted-A}
% \end{equation}
% Here $\mathcal{S}$ denotes the set of system tokens, 
% and $\mathbf{M}^{\mathrm{sup}}_{l,h}$ is a binary indicator mask defined analogously to 
% $\mathbf{M}^{\mathrm{enh}}_{l,h}$ in Eq.~\eqref{eq:mul-enh}. 
% While the uniform shift above assigns the same bias to all image tokens, 
% different visual tokens can carry different levels of semantic importance. 
% To capture this variation, we introduce a similarity-aware bias that adapts the enhancement 
% according to the relevance between the current query and each image token. 
% Specifically, for a query $\mathbf{Q}_{l,h}(i,:)$ and an image key $\mathbf{K}_{l,h}(j,:)$, we compute:
% \begin{equation}
% \matS_{l,h}(i,j) = \max\!\big(0,\;\langle \mathbf{Q}_{l,h}(i,:),\,\mathbf{K}_{l,h}(j,:)\rangle\big),
% \quad i\in\mathcal{T},\; j\in\mathcal{V}.
% \end{equation}
% The resulting score is normalized by a sigmoid function, 
% $\W_{l,h}(i,j) = \sigma\!\big(\matS_{l,h}(i,j)\big)$, 
% which maps it into $(0,1)$ and serves as an adaptive coefficient for weighting the visual tokens. 
% These adaptive weights $\W_{l,h}(i,j)$ allow the model to strengthen more relevant image tokens 
% while assigning weaker biases to less informative ones. 
% The shifted attention logits are then given by
% \begin{equation}
% \tilde{\mathbf{A}}_{l,h}(i,j) =
% \mathbf{A}_{l,h}(i,j) + \hat{\alpha} \, \W_{l,h}(i,j)\!\circ\mathbf{M}^{\mathrm{enh}}_{l,h}(i,j), \quad  i\in \mathcal{T}, j\in \mathcal{V},
% \label{eq:adaptive-shift}
% \end{equation}








% Following the attention calibration described in Section~\ref{sec:attention}, the feedforward netwrok (FFN)通常为两层 fully connected layers with non-
% linear activation 接在attention 后面，并且可以表示为：
% % \begin{equation}
%     \operatorname{FFN}({\matH})=\phi(\left({\matH} {\W}_1\right){\W}_2^{\top},
% \end{equation}
% where $\phi$ is activation function and $\matH$ denotes the xxxx. From the shallow to the deep layers
% of the Transformer, attention is progressively biased towards
% textual tokens, resulting in visual tokens at the deeper layer
% that hardly affect the results. At hence the common stategy is to  reinjecting the visual tokens into the FFN, FFN at l-th layer can be written as follows:
% % Direct updates without introducing extra variables
% \begin{equation}
%   \widetilde{\mathbf{W}}_1^{\top}
%   = \mathbf{W}_1^{\top}
%     + \cos_F(\mathbf{V},\mathbf{W}_1^{\top})\,\mathbf{V},
%   \qquad
%   \widetilde{\mathbf{W}}_2
%   = \mathbf{W}_2
%     + \cos_F(\mathbf{V}^{\top},\mathbf{W}_2)\,\mathbf{V}^{\top}.
% \end{equation}

% \begin{equation}
%   \widetilde{\mathrm{FFN}}(\mathbf{H})
%   = \phi\!\left(\mathbf{H}\,\widetilde{\mathbf{W}}_1\right)\,
%     \widetilde{\mathbf{W}}_2^{\top}.
% \end{equation}


% % Frobenius cosine similarity (used as the scale)
% \begin{equation}
%   \cos_F(\mathbf{A},\mathbf{B})
%   = \frac{\langle \mathbf{A},\mathbf{B}\rangle_F}{\|\mathbf{A}\|_F\,\|\mathbf{B}\|_F},
%   \qquad
%   \langle \mathbf{A},\mathbf{B}\rangle_F = \mathrm{tr}\!\big(\mathbf{A}^{\top}\mathbf{B}\big).
% \end{equation}


% Adapted FFN in the same style


% \begin{equation}
% \W_{l,h}(i,j) = \sigma\!\big(\matS_{l,h}(i,j)\big),
% \end{equation}
% While the uniform shift in Eq.~\eqref{eq:shifted-A} assigns the same bias to all image tokens, 
% different visual tokens carry varying semantic importance. 
% To provide adaptive enhancement, we introduce a similarity-aware bias that modulates the strength 
% according to the relevance between the current query and each image token. 
% Concretely, for a query $\mathbf{q}_{l,h}(i,:)$ and an image key $\mathbf{k}_{l,h}(j,:)$, we compute
% \begin{equation}
% S_{l,h}(i,j) = \max\!\big(0,\;\langle \mathbf{q}_{l,h}(i,:),\,\mathbf{k}_{l,h}(j,:)\rangle\big),
% \quad i\in\mathcal{T},\; j\in\mathcal{V},
% \end{equation}





% The nonnegative similarity is then mapped into $(0,1)$ by a sigmoid gate$
% \W_{l,h}(i,j) = \sigma\!\big(\gamma\, \S_{l,h}(i,j)\big)$
% This adaptive weight $\W_{l,h}(i,j)$ modulates the additive bias for image columns, resulting in
% \begin{equation}
% \tilde{\mathbf{A}}_{l,h}(i,j) =
% \begin{cases}
% \mathbf{A}_{l,h}(i,j) + \beta\, \W_{l,h}(i,j), & i\in \mathcal{T}, j\in \mathcal{V},\\[3pt]
% \mathbf{A}_{l,h}(i,j) + \alpha, & i\in \mathcal{T}, j\in \mathcal{S},\\[3pt]
% \mathbf{A}_{l,h}(i,j), & \text{otherwise}.
% \end{cases}
% \label{eq:adaptive-shift}
% \end{equation}



% To selectively amplify attention toward image tokens, we introduce an additive bias
% based on query–image similarity. To avoid negative enhancement, we optionally apply a rectifier, and then map the score into $(0,1)$ via a sigmoid gate:
% \begin{equation}
% \mathbf{S}_{l,h}(i,j)=\max\!\big(0,\;\langle {\mathbf{Q}}_{l,h}(i,:),\,{\mathbf{K}}_{l,h}(j,:)\rangle\big),
% \quad
% \W_{l,h}(i,j)
% =\sigma(\mathbf{S}_{l,h}(i,j)),
% \;\; j\in\mathcal{V},
% \label{eq:adaptive-weights}
% \end{equation}

% $\mathcal{S}$ is the set of system tokens.
% For earlier queries ($i<|\mathcal{T}|+|\mathcal{V}|$), the same bias is applied to
% all rows without slicing:
% \begin{equation}
% \tilde{\mathbf{A}}_{l,h,i,j} =
% \begin{cases}
% \mathbf{A}_{l,h}(i,j) + \beta \W_{l,h}(i,j), & j\in \mathcal{V},\\[3pt]
% \mathbf{A}_{l,h}(i,j) + \alpha, & j\in \mathcal{S},\\[3pt]
% \mathbf{A}_{l,h}(i,j) & \text{otherwise}.
% \end{cases}
% \end{equation}











% \input{2026_ICLR/figures/framework}


% \subsection{malicious semantics detection}\label{}

% LVLMs typically comprise three core components: a visual
% encoder, a projector, and a language decoder. During the
% reasoning process, the visual encoder encodes user-provided
% images into image tokens, which are subsequently mapped
% to the textual representation space via the projector. These
% image tokens are then concatenated with text tokens and fed
% into the language decoder to generate the corresponding responses.

% When generating the k-th token, the input text XT =
% [xt1
% , xt2
% , . . . , xtT
% ], image XV = [xv1
% , xv2
% , . . . , xvV
% ], and
% historically generated information XH are fed into the language decoder. 

% from the shallow to the deep layers
% of the Transformer, attention is progressively biased towards
% textual tokens, resulting in visual tokens at the deeper layer
% that hardly affect the results,

% models fail to fully utilize visual information, resulting in an excessive dependence on language priors.

% the model demonstrates inadequate attention to the visual modality.

% MLLMs被指出对视觉信息利用不充分~\citep{}是产生幻觉的主要问题，尤其是新visual input和textual input融合后，在解码过程中from the shallow to the deep layers
% of the Transformer, attention is progressively biased towards
% textual tokens, resulting in visual tokens at the deeper layer
% that hardly affect the results,，是产生幻觉的主要原因。

% 我们的方法聚焦在多模态模型的解码过程。When generating the k-th token, the input text XT =
% [xt1
% , xt2
% , . . . , xtT
% ], image XV = [xv1
% , xv2
% , . . . , xvV
% ], and
% historically generated information XH are fed into the language decoder,  predominantly composed of nL transformer blocks with the multi-head self-attention mechanism, where the attention mechanism of the decoder plays
% a pivotal role in integrating visual and textual information.





% We define each block to contain
% nH heads, and the self-attention operation of the h-th head
% in the l-th layer can be formulated as follows:
% \begin{equation}
%     \mathbf{A}_{l,h}=\frac{\mathbf{Q}_{l,h}\mathbf{K}_{l,h}^{\top}}{\sqrt{d_k}}
%     \label{eq1}
% \end{equation}
% \begin{equation}    
% \mathbf{O}_{l,h}=\text{softmax}(\mathbf{A}_{l,h})\mathbf{V}_{l,h}
%     \label{eq2}
% \end{equation}

% In the $l$-th layer transformer block, each attention head $h$ is associated with its own queries $\mathbf{Q}_{l,h}$, keys $\mathbf{K}_{l,h}$, and values $\mathbf{V}_{l,h}$, $\mathbf{Q}_{l,h},\mathbf{K}_{l,h},\mathbf{V}_{l,h}\in\mathbb{R}^{n \times d_k}$, where $n$ represents the length of the input sequence and $d_k$ denotes the dimension of the hidden state. The attention matrix $\mathbf{A}_{l,h}\in \mathbb{R}^{n \times n}$ is computed as the product of queries $\mathbf{Q}_{l,h}$ and keys $\mathbf{K}_{l,h}$。我们的目的是增强对视觉token注意力的得分，最直接的做法是对注意力矩阵中的元素加一个值：
% \begin{equation}
% \hat{Z}_{l,h} = Z_{l,h} + \alpha \cdot M^{enh}_{l,h} \circ Z_{l,h}
% \end{equation}，
% where $\alpha$ is the enhancement coefficient ($\alpha>0$),$M_{l, h}^{enh}(i, j) = \mathbb{I}(i \in \mathcal{T}, j \in \mathcal{V})$是增强矩阵。但是这样会有一个问题，乘 >1 会把正的logits 放大（softmax 后概率更大），但如果某些 logits 本来是负的，乘 >1 会更负，反而更小, 与“增强”初衷可能相反。对目标列 logit += log(倍率)，在 softmax 里严格等价于把该列概率乘以这个倍率（再归一化），不管原来是正是负，效果都朝你想要的方向走。


% Sb,h,i,j​=max(0,⟨Q^​b,h,i​,K^b,h,j​⟩),Wb,h,i,j​=t=img_s∑img_e−1​exp(Sb,h,i,t​/τ)exp(Sb,h,i,j​/τ)​,τ=0.5.

% β=ln(enh_para)=ln(self.enh_para),α=ln(sup_para)=ln(self.sup_para).

% AttnProbsb,h,i,:​=softmax(Lb,h,i,:′​),Outb,h,i​=j=0∑K−1​AttnProbsb,h,i,j​Vb,h,j​.



% We enhance multimodal large language models (MLLMs) by adaptively amplifying the attention scores assigned to image tokens in the decoder layers. Consider the $l$-th transformer block with $n_H$ heads. The self-attention computation of the $h$-th head is formulated as:
% \begin{equation}
% \mathbf{A}_{l,h} = \frac{\mathbf{Q}_{l,h}\mathbf{K}_{l,h}^{\top}}{\sqrt{d_k}},
% \quad
% \mathbf{O}_{l,h} = \text{softmax}(\mathbf{A}_{l,h}) \mathbf{V}_{l,h},
% \label{eq:attention}
% \end{equation}
% where $\mathbf{Q}_{l,h}, \mathbf{K}_{l,h}, \mathbf{V}{l,h}\in\mathbb{R}^{n\times d_k}$ denote query, key, and value matrices, with $n$ the sequence length and $d_k$ the hidden dimension. The attention matrix $\mathbf{A}{l,h}\in\mathbb{R}^{n\times n}$ captures the similarity between tokens.

% To encourage stronger focus on visual tokens, a straightforward approach is to enhance the corresponding logits in $\mathbf{A}{l,h}$:
% \begin{equation}
% \hat{\A}_{l,h} = Z_{l,h} + \alpha \cdot M^{\mathrm{enh}}_{l,h} \circ \A_{l,h},
% \end{equation}
% where $M^{\mathrm{enh}}_{l,h}(i,j)=\mathbb{I}(i \in \mathcal{T}, j \in \mathcal{V})$ selects query–key pairs between text tokens $\mathcal{T}$ and image tokens $\mathcal{V}$, and $\alpha>0$ is a fixed enhancement coefficient. However, this naive multiplicative scaling introduces an inconsistency: positive logits are enlarged, but negative logits are pushed further negative, thereby reducing their contribution after the softmax normalization. This effect contradicts the intended goal of consistently enhancing visual attention.

% To resolve this, we adopt a logit-shifting strategy that operates in the probability space. Specifically, scaling the $j$-th column probability in softmax by a factor $r>1$ is strictly equivalent to adding $\log(r)$ to the corresponding logits before normalization. Formally,
% \begin{equation}
% \tilde{\A}_{l,h}(i,j) =
% \begin{cases}
% \A_{l,h}(i,j) + \beta, & j \in \mathcal{V},\
% \A_{l,h}(i,j) + \alpha, & j \notin \mathcal{V},
% \end{cases}
% \end{equation}
% where $\beta=\ln(\texttt{enh_para})$ and 

% $\alpha=\ln(\texttt{sup_para})$ denote adaptive enhancement and suppression terms, respectively. This formulation guarantees that amplification always increases the relative probability mass of image tokens in $\text{softmax}(\tilde{\A}_{l,h})$, independent of the sign of the original logits.

% The final attention distribution is then computed as
% \begin{equation}
% \text{AttnProbs}{b,h,i,:} = \text{softmax}\big(\tilde{Z}{b,h,i,:}/\tau\big),
% \quad
% \mathbf{O}{b,h,i} = \sum{j=0}^{n-1} \text{AttnProbs}{b,h,i,j},\mathbf{V}{b,h,j},
% \end{equation}
% with temperature $\tau=0.5$ to stabilize the adjustment. This design adaptively amplifies attention toward visual tokens while mitigating the sign inconsistency issue inherent in naive scaling.



% \paragraph{Adaptive logit shifting.}
% To selectively amplify attention toward image tokens, we introduce an additive bias
% based on query–image similarity. Let $\beta=\ln(\texttt{enh\_para})>0$ denote the
% enhancement strength, and $\alpha=\ln(\texttt{sup\_para})<0$ denote the suppression
% strength for system tokens. For each query $\mathbf{q}_{b,h,i}$ and image key
% $\mathbf{k}_{b,h,j}$, define normalized representations
% \begin{equation}
% \widehat{\mathbf{q}}_{b,h,i} = 
% \frac{\mathbf{q}_{b,h,i}}{\|\mathbf{q}_{b,h,i}\|_2}, 
% \qquad
% \widehat{\mathbf{k}}_{b,h,j} = 
% \frac{\mathbf{k}_{b,h,j}}{\|\mathbf{k}_{b,h,j}\|_2}.
% \end{equation}
% Their cosine similarity is
% \begin{equation}
% s_{b,h,i,j} = 
% \left\langle \widehat{\mathbf{q}}_{b,h,i},\,\widehat{\mathbf{k}}_{b,h,j}\right\rangle,
% \quad j\in\mathcal{V}.
% \end{equation}
% To avoid negative enhancement, we optionally apply a rectifier $s'_{b,h,i,j}=\max(0,s_{b,h,i,j})$,
% and then map the score into $(0,1)$ via a sigmoid gate:
% \begin{equation}
% w_{b,h,i,j} = \sigma(\gamma \, s'_{b,h,i,j}),
% \qquad 
% \sigma(x) = \frac{1}{1+e^{-x}},\;\;\gamma=6.0.
% \end{equation}

% The attention logits are shifted as follows.  
% For queries beyond the image prefix ($i \geq |\mathcal{T}|+|\mathcal{V}|$):
% \begin{equation}
% \tilde{\mathbf{A}}_{b,h,i,j} =
% \begin{cases}
% \mathbf{A}_{b,h,i,j} + \beta \, w_{b,h,i,j}, & j\in \mathcal{V},\\[3pt]
% \mathbf{A}_{b,h,i,j} + \alpha, & j\in \mathcal{S},\\[3pt]
% \mathbf{A}_{b,h,i,j}, & \text{otherwise},
% \end{cases}
% \end{equation}
% where $\mathcal{S}$ is the set of system tokens.
% For earlier queries ($i<|\mathcal{T}|+|\mathcal{V}|$), the same bias is applied to
% all rows without slicing:
% \begin{equation}
% \tilde{\mathbf{A}}_{b,h,i,j} =
% \begin{cases}
% \mathbf{A}_{b,h,i,j} + \beta \, w_{b,h,i,j}, & j\in \mathcal{V},\\[3pt]
% \mathbf{A}_{b,h,i,j} + \alpha, & j\in \mathcal{S},\\[3pt]
% \mathbf{A}_{b,h,i,j}, & \text{otherwise}.
% \end{cases}
% \end{equation}

% Finally, the modified attention distribution and output are
% \begin{equation}
% \operatorname{AttnProbs}_{b,h,i,:}
% =\softmax\!\big(\tilde{\mathbf{A}}_{b,h,i,:}/\tau\big), 
% \qquad
% \mathbf{O}_{b,h,i}
% =\sum_{j=0}^{n-1}\operatorname{AttnProbs}_{b,h,i,j}\,\mathbf{V}_{b,h,j},
% \end{equation}
% with $\tau=0.5$ for stability.
% This design introduces adaptive, similarity-aware enhancement for image tokens while
% suppressing system tokens, ensuring stable biasing of attention without sign inconsistency.




% With temperature $\tau>0$ (default $\tau=0.5$), the attention distribution and head output are
% \begin{align}
% \operatorname{AttnProbs}_{b,h,i,j}
% &= \frac{\exp\!\big(\tilde{\mathbf{A}}_{b,h,i,j}/\tau\big)}
% {\displaystyle \sum_{t=0}^{n-1}\exp\!\big(\tilde{\mathbf{A}}_{b,h,i,t}/\tau\big)},
% \qquad
% \label{eq:attnprobs}
% \\[4pt]
% \mathbf{O}_{b,h,i}
% &= \sum_{j=0}^{n-1} \operatorname{AttnProbs}_{b,h,i,j}\,\mathbf{V}_{b,h,j}.
% \label{eq:head-out}
% \end{align}

% \paragraph{Why shifting works.}
% For any fixed query $(b,h,i)$ and any key index $j^\star$, adding a constant $\Delta$ to the $j^\star$-th logit is equivalent to multiplying the corresponding softmax probability by $e^{\Delta/\tau}$ followed by renormalization:
% \begin{equation}
% \softmax\big(\mathbf{z}+\Delta\,\mathbf{e}_{j^\star}\big)_{j}
% =
% \frac{e^{\Delta}\,e^{z_{j^\star}}}{\sum_{t} e^{z_t} + \big(e^{\Delta}-1\big) e^{z_{j^\star}}}\;\I(j=j^\star)
% +\;\frac{e^{z_{j}}}{\sum_{t} e^{z_t} + \big(e^{\Delta}-1\big) e^{z_{j^\star}}}\;\I(j\neq j^\star).
% \label{eq:softmax-shift-lemma}
% \end{equation}
% Hence $\beta>0$ increases the relative probability mass of image tokens \emph{regardless of the original logit sign}, while $\alpha<0$ gently deflates non-image mass to maintain calibration.

% \paragraph{Optional: adaptive enhancement within image tokens.}
% To further concentrate mass on visually relevant regions, define normalized query/key features
% $\widehat{\mathbf{Q}}=\mathrm{normalize}(\mathbf{Q},\text{dim}=-1)$,
% $\widehat{\mathbf{K}}=\mathrm{normalize}(\mathbf{K},\text{dim}=-1)$,
% and a nonnegative similarity
% \begin{equation}
% S_{l,h}(i,j)=\max\!\big(0,\;\langle \widehat{\mathbf{Q}}_{b,h,i,:},\,\widehat{\mathbf{K}}_{b,h,j,:}\rangle\big),
% \quad
% W_{b,h,i,j}
% =\frac{\exp\!\big(S_{b,h,i,j}/\tau_s\big)}{\displaystyle\sum_{t\in\mathcal{V}}\exp\!\big(S_{b,h,i,t}/\tau_s\big)},
% \;\; j\in\mathcal{V},
% \label{eq:adaptive-weights}
% \end{equation}
% with a small temperature $\tau_s$ (e.g., $0.5$). Replace the uniform column shift $\beta$ in \eqref{eq:shifted-A} by a token-wise shift $\beta\,W_{b,h,i,j}$ for $j\in\mathcal{V}$. This keeps the guarantee in \eqref{eq:softmax-shift-lemma} while adaptively prioritizing more relevant image tokens.

% \paragraph{Complexity and implementation.}
% Eq.~\eqref{eq:shifted-A} adds only a column-wise bias over keys (two scalars $\alpha,\beta$ or an image-key mask plus a per-query weighting in the adaptive variant). No change to value aggregation \eqref{eq:head-out} or cache formats is required, and the memory/compute overhead is negligible relative to the baseline attention.



            % # 计算对每个图像token的自适应偏置：sim(Q, K_img)，并用加法偏置更稳定
            % beta  = math.log(self.enh_para)  # >0 时增强强度
            % alpha = math.log(self.sup_para)  # <0 时抑制系统列（sup_para<1 常用）

            % # 归一化后做余弦相似度：sim ∈ [-1, 1]，形状 (B, H, q_len, IMG_LEN)
            % Qn     = F.normalize(query_states, dim=-1, eps=1e-6)
            % Kn_img = F.normalize(key_states[:, :, SYS_LEN:SYS_LEN+IMG_LEN, :], dim=-1, eps=1e-6)
            % sim    = torch.matmul(Qn, Kn_img.transpose(-1, -2))                         # (B,H,q_len,IMG_LEN)
            % # 若只想“增强”而不减弱，可解开下一行：只保留正相似度
            % sim = F.relu(sim)
            % w = torch.sigmoid(6.0 * sim)   

            % if q_len > SYS_LEN + IMG_LEN:
            %     # 仅对“图像之后的文本 query 行”生效（保持你原来的行切片逻辑）
            %     attn_weights[:, :, SYS_LEN+IMG_LEN:, SYS_LEN:SYS_LEN+IMG_LEN] += beta * w[:, :, SYS_LEN+IMG_LEN:, :]
            %     attn_weights[:, :, SYS_LEN+IMG_LEN:, :SYS_LEN]                += alpha
            % else:
            %     # 还在系统+图像前缀阶段：对所有 query 行生效（与你原逻辑一致）
            %     attn_weights[:, :, :, SYS_LEN:SYS_LEN+IMG_LEN] += beta * w
            %     attn_weights[:, :, :, :SYS_LEN]                += alpha


%===========================================
% 一眼看懂的小例子

% 原 logits（某个 query 的三列）：[2.0, -0.1, -1.0]
% 想把第 2 列“增强一倍”。

% 乘法（×2）：[2.0, -0.2, -1.0]

% 原来第 2 列概率 ≈ e^-0.1 / (e^2 + e^-0.1 + e^-1) ≈ 0.104

% 乘法后第 2 列概率 ≈ 0.095（反而更小）

% 加法（+log 2）：[2.0, -0.1 + 0.693, -1.0] = [2.0, 0.593, -1.0]

% 第 2 列概率 ≈ 0.189（确实变大）

% 同理，抑制时用 log(小于1) 会稳定变小，不会像乘法那样把负数“抬高”。
%+========================================


% Multimodal large language models (MLLMs) often produce harmful responses when exposed to malicious prompts or unsafe visual inputs. Prior work attributes this vulnerability to the \emph{continuous nature of visual token embeddings}~\citepp{eta}, which deviate from the discrete textual embeddings and thereby bypass safety mechanisms originally designed for language backbones~\citepp{COCA, MLLM-Protector, ShiftDC, DTR}. As illustrated in Fig.~\ref{}, visual and textual representations remain poorly aligned, highlighting the risk that harmful semantics in images may be overlooked.  

% This motivates the need for explicitly modeling the correlation between visual inputs and unsafe semantics. To this end, we define a set of $C$ unsafe prompt categories (listed in Appendix), denoted as $\mathcal{Z} = \{z_i\}_{i=1}^{C}$. These prompts serve as semantic anchors to measure the similarity between an input image and potentially harmful content. Concretely, we employ the CLIP model~\citepp{clip} to encode an input image $x$ and a textual prompt $z$ into their respective feature representations:
% \begin{equation}
%     \mathbf{x} = \Phi_v(x), \quad \mathbf{z} = \Phi_t(z),
% \end{equation}
% where $\Phi_v(\cdot)$ and $\Phi_t(\cdot)$ denote the image and text encoders. While CLIP aligns images and texts in a shared feature space, global image embeddings often include irrelevant semantics (e.g., background), reducing alignment accuracy. We thus adopt a fine-grained modeling: each image is divided into $M$ patches $\{x^m\}_{m=1}^M$ with features $\{\mathbf{x}^m\}_{m=1}^M$, and each prompt $z_i$ is expanded into $N$ textual variants, yielding $\{\mathbf{z}_i^n\}_{n=1}^N$.  
% We model the image and prompts as discrete distributions:
% \begin{equation}
%     \mathbb{P}(\x) = \sum_{m=1}^{M} a^m \delta(\mathbf{x}^m-\x), \quad 
%     \mathbb{Q}_i(\z) = \sum_{n=1}^{N} b_i^n \delta(\mathbf{z}_i^n-\z),
% \end{equation}
% where $\delta(\cdot)$ is the Dirac delta function, and $a^m$, $b_i^n$ are importance weights. For image patches, we assign $a^m$ according to entropy with respect to the average prompt embedding $\bar{\mathbf{z}}_i = \frac{1}{N}\sum_{n=1}^N \mathbf{z}_i^n$:
% \begin{equation}
%     a^m = \frac{\exp(h(\mathbf{x}^m))}{\sum_{m'} \exp(h(\mathbf{x}^{m'}))}, \quad 
%     h(\mathbf{x}^m) = -\sum_{i=1}^C p(\bar{\mathbf{z}}_i|\mathbf{x}^m)\log p(\bar{\mathbf{z}}_i|\mathbf{x}^m).
% \end{equation}
% Low-entropy patches (more confident predictions) are assigned higher weights. Textual weights $b_i^n$ are computed analogously.  
% Given $\mathbb{P}(\x)$ and $\mathbb{Q}_i(\z)$, we measure their alignment via OT distance:
% \begin{equation}
%     d_{\mathrm{OT}}(\mathbb{P}, \mathbb{Q}_i; \mathbf{C}_i) 
%     = \min_{\mathbf{T}_i \ge 0} \langle \mathbf{T}_i, \mathbf{C}_i \rangle, 
%     \quad \text{s.t.} \quad \mathbf{T}_i \mathbf{1}_M = \mathbf{a}, \; 
%     \mathbf{T}_i^\top \mathbf{1}_N = \mathbf{b}_i,
% \end{equation}
% where $\mathbf{a}=[a^1,\dots,a^M]^\top$, $\mathbf{b}_i=[b_i^1,\dots,b_i^N]^\top$, and $\mathbf{C}_i(m,n)=1-\cos(\mathbf{x}^m,\mathbf{z}_i^n)$. The transport plan $\mathbf{T}_i$ can be efficiently obtained via the Sinkhorn-Knopp algorithm~\citepp{sinkhorn}.
% A lower OT distance indicates a closer alignment with harmful semantics, providing a quantitative measure for detecting unsafe content.



% \subsection{Masking-guided Alignment}
% The OT distance introduced in Section~\ref{sec:ot_cal} not only serves as a criterion for unsafe-content detection, but also decomposes into patch-level contributions that indicate which regions are most associated with harmful semantics. To capture this information, we assign each image patch $m$ an aggregated OT score by summing its transport contributions over all unsafe prompt categories:
% \begin{align}
%     d_{\mathrm{OT}}(m) &= \sum_{i=1}^{C}\sum_{n=1}^{N}\mathbf{T}_i(m,n)\,\mathbf{C}_i(m,n), \label{eq:dotm}
% \end{align}
% where $\mathbf{T}_i(m,n)$ denotes the transport mass from image patch $m$ to the $n$-th textual variant of category $i$.
% $d_{\mathrm{OT}}(m)$ quantifies the contribution of patch $m$ to the OT objective and thereby captures its association with unsafe semantics: smaller values indicate closer alignment to harmful prompts, whereas larger values imply weaker correlation. Based on these patch-level OT distances, we determine unsafe-associated regions by thresholding:
% \begin{align}
%     \mathcal{S}_{\text{unsafe}} = \{\, m \mid d_{\mathrm{OT}}(m) \le \tau \,\}.
% \end{align}
% We then construct a sanitized visual input by masking the patches in $\mathcal{S}_{\text{unsafe}}$:
% \begin{align}
%     \hat{x}^m =
%     \begin{cases}
%         0,   & m \in \mathcal{S}_{\text{unsafe}}, \\
%         x^m, & \text{otherwise},
%     \end{cases}
%     \qquad
%     \hat{x}=\{\hat{x}^m\}_{m=1}^M,
% \end{align}
% which suppresses unsafe cues while retaining benign context for subsequent reasoning. To further bias the generation process toward safe completions, we prepend a lightweight safety-aware prefix (e.g., ``As an AI assistant, ...'') to the user prompt. This prefix activates the intrinsic safety mechanisms of MLLMs and steers the model toward responsible outputs. The resulting generation process is defined as:
% \begin{equation}
%     y_t \sim \pi_\theta\!\left(\cdot \,\middle|\, G\!\big(\Phi(\hat{x})\big),\, \mathcal{P},\, y_{<t}\right), \quad t=1,\dots,T,
% \end{equation}
% where $\hat{x}$ is the masked visual input and $\mathcal{P}$ is the prefix-augmented textual prompt. In practice, the threshold $\tau$ is set adaptively as the $q$-quantile of $\{d_{\mathrm{OT}}(m)\}_{m=1}^M$, which is equivalent to masking the top-$K$ patches with $K=\lfloor qM\rfloor$. Here, $q \in (0,1)$ is a hyperparameter that controls the masking ratio: a smaller $q$ masks fewer patches, whereas a larger $q$ masks more patches. To avoid degenerate cases, the masking ratio is further clipped within $[q_{\min}, q_{\max}]$.




% \subsection{Theoretical Analysis}
% To establish the efficacy of our OT-based method for detecting unsafe patches in multimodal content, we analyze the expected \emph{distance} gap between pairs of patches. We compare the OT-based distance \(d_{\mathrm{OT}}(m)\) with a cosine-based distance baseline $
% d_{\cos}(m)\;=\;\sum_{i=1}^{C}\sum_{n=1}^{N}\bigl(1-\cos(\mathbf{x}^m,\mathbf{z}_i^n)\bigr),
% $. Both measures share the same direction (larger distance \(\Rightarrow\) weaker alignment with unsafe prompts). For patches \(m_1\in\mathcal{S}_{\text{unsafe}}\) and \(m_2\in\mathcal{S}_{\text{safe}}\), we show that the OT-based method yields a larger expected distance gap:
% \begin{equation}
% \mathbb{E}[|d_{\mathrm{OT}}(m_2) - d_{\mathrm{OT}}(m_1)|] > \mathbb{E}[|d_{\cos}(m_1) - d_{\cos}(m_2)|].
% \end{equation}
% \paragraph{Why OT enlarges the distance gap.}
% The OT-based method leverages global distribution alignment with capacity constraints and entropy-based weights. The transport plan \( \mathbf{T}_i \) prioritizes low-cost pairs for unsafe patches, assigning lower \( d_{\mathrm{OT}}(m) \), while safe patches yield higher values due to weaker alignment. Conversely, \( d_{\cos}(m) \) averages all pairwise costs, including irrelevant semantics, reducing the gap. This amplification enables robust threshold-based classification (Section~\ref{sec:ot_cal}). A formal proof, using a product-coupling baseline, is in Appendix~\ref{proof:score_diff}.





% \subsection{Theoretical Analysis}
% To establish the efficacy of our OT-based method for detecting unsafe patches in multimodal content, we analyze the expected \emph{distance} difference between pairs of patches. Specifically, we compare the OT-based distance \(d_{\mathrm{OT}}(m)\) against a cosine-based distance baseline
% $
% d_{\cos}(m) \;=\; \sum_{i=1}^{C} \sum_{n=1}^{N} \bigl(1-\cos(\mathbf{x}^m, \mathbf{z}_i^n)\bigr),
% $
% which aligns the direction of both measures (larger distance \(\Rightarrow\) less aligned with unsafe prompts). For patches \(m_1 \in \mathcal{S}_{\text{unsafe}}\) and \(m_2 \in \mathcal{S}_{\text{safe}}\), we prove that the OT-based method yields a larger expected distance gap:
% \begin{equation}
% \mathbb{E}[|d_{\mathrm{OT}}(m_2) - d_{\mathrm{OT}}(m_1)|] > \mathbb{E}[|d_{\cos}(m_1) - d_{\cos}(m_2)|].
% \end{equation}
% \paragraph{Why OT enlarges the distance gap.}
% The superiority of the OT-based approach stems from its ability to model the \emph{global} alignment between the patch and prompt distributions under marginal (capacity) constraints, together with entropy-based weighting. The optimal transport plan concentrates mass on truly relevant text variants and, when popular variants are congested, pushes excess mass to higher-cost alternatives. In contrast, the cosine-based distance \(d_{\cos}(m)\) aggregates all pairwise terms uniformly, including irrelevant or noisy contributions (e.g., background semantics), which dilutes the distinction between safe and unsafe patches. As a consequence, unsafe patches (more aligned with harmful prompts) receive consistently lower \(d_{\mathrm{OT}}(m)\), while safe patches receive higher values, producing a larger expected gap as in~\eqref{eq:ot-vs-cos}. A formal derivation via a product-coupling baseline and a capacity-induced amplification term is provided in Appendix~\ref{proof:score_diff}.

% \paragraph{Implication for thresholding and masking.}
% This amplified distance gap directly supports our masking-guided alignment strategy: patches with \(d_{\mathrm{OT}}(m) \le \tau\) are identified as unsafe and masked to suppress harmful semantics, while the remaining patches are retained for reasoning. The enhanced separability ensures that the threshold \(\tau\)—set adaptively as the \(q\)-quantile of \(\{d_{\mathrm{OT}}(m)\}_{m=1}^M\) (Section~\ref{sec:ot_cal})—reliably distinguishes unsafe regions, thereby improving the safety of the MLLM’s generated outputs without sacrificing benign context.






% To establish the efficacy of our OT-based method for detecting unsafe patches in multimodal content, we analyze the expected score difference between pairs of patches. Specifically, we compare the OT-based distance, defined as $d_{\mathrm{OT}}(m)$, against the baseline similarity-based distance, $ s(m) = \sum_{i=1}^{C} \sum_{n=1}^{N} \cos(\mathbf{x}^m, \mathbf{z}_i^n) $. For patches $ m_1 \in \mathcal{S}_{\text{unsafe}} $ and $ m_2 \in \mathcal{S}_{\text{safe}} $, we prove that the OT-based method yields a larger expected score difference:
% \begin{equation}
% \mathbb{E}[|d_{\mathrm{OT}}(m_2) - d_{\mathrm{OT}}(m_1)| \mid m_1 \in \mathcal{S}_{\text{unsafe}}, m_2 \in \mathcal{S}_{\text{safe}}] > \mathbb{E}[|s(m_1) - s(m_2)|],
% \end{equation}
% facilitating more robust threshold-based classification. 
% % Explaining why OT is superior
% The superiority of the OT-based approach stems from its ability to model the global alignment between patch and prompt distributions, leveraging entropy-based weights and optimal transport plans to prioritize semantically relevant patch-prompt pairs. This contrasts with the cosine similarity score, which aggregates all pairwise similarities equally, including irrelevant or noisy contributions (e.g., background semantics), thus diluting the distinction between safe and unsafe patches. By amplifying the score difference, our method ensures that unsafe patches (with stronger alignment to harmful prompts) are assigned lower $ d_{\mathrm{OT}}(m)$ scores, while safe patches receive higher scores, enabling a clearer separation via a threshold $\tau$ (as defined in Section~\ref{sec:ot_cal}). The complete proof is provided in Appendix~\ref{proof:score_diff}.
% % Connecting to the masking-guided alignment
% This larger score difference directly supports our masking-guided alignment strategy, where patches with \( d_{\mathrm{OT}}(m) \leq \tau \) are identified as unsafe and masked to suppress harmful semantics. The enhanced separability ensures that the threshold \( \tau \), set as the \( q \)-quantile of \( \{d_{\mathrm{OT}}(m)\}_{m=1}^M \), reliably distinguishes unsafe regions, thereby improving the safety of the MLLM's generated outputs.



% To demonstrate the superiority of our optimal transport (OT)-based scoring method in distinguishing between safe and unsafe patches, we analyze the expected score difference between pairs of patches. Specifically, we compare the OT-based score $ d_{\mathrm{OT}}(m) $ against the cosine similarity-based score $ s(m) = \sum_{i=1}^{C} \sum_{n=1}^{N} \cos(\mathbf{x}^m, \mathbf{z}_i^n) $. For patches $ m_1 \in \mathcal{S}_{\text{unsafe}} $ and $ m_2 \in \mathcal{S}_{\text{safe}} $, we prove that the OT-based method yields a larger expected score difference:
% \begin{equation}
%      \mathbb{E}[|d_{\mathrm{OT}}(m_2) - d_{\mathrm{OT}}(m_1)|] > \mathbb{E}[|s(m_1) - s(m_2)|] ,
% \end{equation}

% facilitating more robust threshold-based classification. This is because OT leverages global distribution matching and entropy-based weighting to amplify the semantic distinction between unsafe and safe patches, while cosine similarity aggregates pairwise similarities without such optimization. The complete proof is provided in Appendix~\ref{proof:score_diff}.

% This result is critical for our multimodal content detection framework, as a larger score difference enhances the separability of safe and unsafe patches, enabling clearer threshold settings for classification tasks, such as identifying harmful content in images.



% A lower OT distance indicates a closer alignment with harmful semantics, providing a reliable criterion for detecting unsafe content. 
% At the same time, the OT formulation decomposes this distance into patch-level contributions, 
% revealing which regions are entangled with unsafe semantics and laying the foundation for our subsequent masking-guided alignment.

% A lower OT distance indicates a closer alignment with harmful semantics, serving as a principled criterion for detecting unsafe content. 
% Beyond detection, the transport plan yields patch-level attributions, enabling us to directly localize harmful regions—an observation that underpins our masking-guided alignment approach.

% A lower OT distance indicates a closer alignment with harmful semantics, offering a principled criterion for unsafe content detection. 
% Crucially, the transport plan also attributes these distances to individual patches, 
% which provides fine-grained cues about where unsafe semantics reside and naturally motivates our masking-guided alignment strategy.

% Multimodal large language models (MLLMs) still tend to produce harmful responses when exposed to malicious prompts or unsafe image inputs. Recent studies reveal that such safety failures mainly stem from the \emph{continuous nature of visual token embeddings}~\citepp{eta}, which deviate significantly from the discrete textual token embeddings. As discussed in prior works~\citepp{COCA, MLLM-Protector, ShiftDC, DTR}, this modality gap enables harmful visual inputs to bypass the safety mechanisms originally established in language backbones. We illustrate examples of such feature discrepancies in Fig.~\ref{}, where textual and visual representations remain clearly separated. These observations suggest that visual inputs are insufficiently aligned with the textual modality. Motivated by this, we propose a novel safety-aware framework that explicitly detects and mitigates malicious semantics, thereby safeguarding both visual and textual information.

% To detect malicious semantics in visual inputs, we define a set of $C$ unsafe prompt categories (listed in Appendix), denoted as $\mathcal{Z} = \{z_i\}_{i=1}^{C}$. These prompts serve as semantic anchors to measure the similarity between an input image and potentially harmful content. Concretely, we employ the CLIP model~\citepp{clip} to encode an input image $x$ and a textual prompt $z$ into their respective feature representations:
% \begin{equation}
%     \mathbf{x} = \Phi_v(x), \quad \mathbf{z} = \Phi_t(z),
% \end{equation}
% where $\Phi_v(\cdot)$ and $\Phi_t(\cdot)$ denote the image and text encoders, respectively. CLIP aligns images and texts into a unified feature space through contrastive learning. However, visual features often capture the entire image semantics, including background and irrelevant objects, which may not align with the predefined unsafe categories. To address this issue, we introduce fine-grained semantic alignment between visual and textual features. Specifically, for each input image, we divide it into $M$ patches $\{x^m\}_{m=1}^{M}$, which are encoded into patch-level features $\{\mathbf{x}^m\}_{m=1}^{M}$. Likewise, for each unsafe prompt $z_i$, we construct $N$ fine-grained textual variants, resulting in a set of features $\{\mathbf{z}_i^{n}\}_{n=1}^{N}$.


% We model each image and class as a discrete distribution, rather than a single embedding. For an image $\hat{x}$ and category $i$, we define their distributions as: 
% \begin{equation} 
%     \mathbb{P}(\x) = \sum_{m=1}^{M} a^m \delta({{\mathbf{x}}^m}-\x), \quad 
%     \mathbb{Q}_i(\z) = \sum_{n=1}^{N} b_i^n \delta({\mathbf{z}_i^n}-\z), 
% \end{equation} 
% where $\delta(\cdot)$ denotes the Dirac delta function, and ${a^m}$, ${b_i^n}$ are the associated importance weights. 
% To compute ${a^m}$ for the divided image feature ${\mathbf{x}}^m$, we assess its entropy with respect to the average prompt embedding $\bar{\mathbf{z}}_i = \frac{1}{N}\sum_{n=1}^N \mathbf{z}_i^n$. Specifically,
% \begin{equation} 
%     a^m = \frac{\exp\left(h({\mathbf{x}}^m)\right)}{\sum_{m'=1}^M \exp\left(h({\mathbf{x}}^{m'})\right)}, 
%     \quad h({\mathbf{x}}^m) = -\sum_{i=1}^C p(\bar{\mathbf{z}}_i|{\mathbf{x}}^m) \log p(\bar{\mathbf{z}}_i|{\mathbf{x}}^m).
% \end{equation} 
% The entropy $h({\mathbf{x}}^m)$ reflects the prediction confidence: features with lower entropy are assigned higher weights. The textual weights ${b_i^n}$ are computed analogously.  

% Given $\mathbb{P}(\x)$ and $\mathbb{Q}_i(\z)$, we measure their alignment using the OT distance, which captures the minimal semantic transport cost between image and text features. The transport plan $\mathbf{T}_{i} \in \mathbb{R}^{M\times N}$ is obtained by solving moves mass from $\mathbb{P}(\x)$ to $\mathbb{Q}_i(\z)$, subject to the marginal constraints: 
% \begin{equation} 
%     d_{\mathrm{OT}}(\mathbb{P}(\x), \mathbb{Q}_i(\z); {\mathbf{C}}_{i}) 
%     = \min_{\mathbf{T}_{i} \ge \mathbf{0}} \langle \mathbf{T}_{i}, \mathbf{C}_{i} \rangle, 
%     \quad \text{s.t.} \quad \mathbf{T}_{i} \mathbf{1}_M = \mathbf{a}, \quad \mathbf{T}_{i}^\top \mathbf{1}_N = \mathbf{b}_i,
% \end{equation}
% where $\mathbf{a} = [a^1, \cdots, a^M]^\top$, $\mathbf{b}_i = [b_i^1, \cdots, b_i^N]^\top$, and $\mathbf{C}_i \in \mathbb{R}^{M \times N}$ denotes the transport cost. We define the cost as following:
% \begin{equation}
%     {\mathbf{C}}_{i}(m, n) = 1 - \cos\left({\mathbf{x}}^m, \mathbf{z}_i^n\right),
% \end{equation}
% where $\cos(\cdot,\cdot)$ denotes cosine similarity.  
% This OT formulation provides a principled measure of the semantic discrepancy between an image and each unsafe category. A lower transport distance indicates a stronger alignment with harmful semantics, which we use as the detection signal for malicious visual inputs.


% \subsection{Masking-guided Alignment}
% The OT distance defined in Section~\ref{sec:ot_cal} not only provides a criterion for unsafe-content detection, but also yields patch-level costs that specify which regions are most associated with harmful semantics. Leveraging this property, we compute a per-patch score by aggregating its contribution to the OT objective across all unsafe prompt categories:
% \begin{align}
%     d_{\mathrm{OT}}(m) &= \sum_{i=1}^{C}\sum_{n=1}^{N}\mathbf{T}_i(m,n)\,\mathbf{C}_i(m,n), \label{eq:dotm}
% \end{align}
% where $\mathbf{T}_i(m,n)$ is the transported mass from image patch $m$ to the $n$-th textual variant of unsafe category $i$, and $\mathbf{C}_i(m,n)=1-\cos(\mathbf{x}^m,\mathbf{z}_i^n)$ is the semantic transport cost. Intuitively, $d_{\mathrm{OT}}(m)$ is the portion of the OT objective attributed to patch $m$; smaller values indicate closer correspondence to unsafe prompts.

% To identify unsafe-associated patches, we apply a threshold:
% \begin{align}
%     \mathcal{S}_{\text{unsafe}} &= \{\, m \mid d_{\mathrm{OT}}(m) \le \tau \,\}
% \end{align}
% We then construct a masked visual input by removing only the implicated patches:
% \begin{align}
%     \hat{x}^m =
%     \begin{cases}
%         0,   & m \in \mathcal{S}_{\text{unsafe}}, \\
%         x^m, & \text{otherwise},
%     \end{cases}
%     \qquad
%     \hat{x}=\{\hat{x}^m\}_{m=1}^M,
% \end{align}
% which suppresses unsafe cues while retaining benign context for downstream reasoning. To bias generation toward safe completions, we prepend a lightweight safety-aware prefix to the user prompt and decode on the masked input:
% \begin{equation}
%     y_t \sim \pi_\theta\!\left(\cdot \,\middle|\, G\!\big(\Phi(\hat{x})\big),\, \mathcal{P},\, y_{<t}\right), \quad t=1,\dots,T,
% \end{equation}
% where $\mathcal{P}$ denotes the prefix-augmented textual prompt.

% In practice, we set the threshold $\tau$ adaptively as the $q$-quantile of $\{d_{\mathrm{OT}}(m)\}_{m=1}^M$, which is equivalent to masking the top-$K$ implicated patches with $K=\lfloor qM\rfloor$. To avoid degenerate cases, the masked ratio is clipped within $[q_{\min}, q_{\max}]$. For models based on patch tokens (e.g., ViT), replacing a masked patch with a learned \emph{mask token} is equivalent to zeroing; we adopt zeroing for simplicity and efficiency. The OT solution $\mathbf{T}_i$ is computed using entropic regularization with the Sinkhorn algorithm, which guarantees fast convergence and yields a total complexity of $\mathcal{O}(C\,M N\,L)$ for $L$ Sinkhorn iterations.


% The OT distance defined in Section~\ref{sec:ot_cal} not only provides a criterion for unsafe-content detection, but also yields patch-level costs that specify which regions are most associated with harmful semantics. Leveraging this property, we compute a per-patch score by aggregating its contribution to the OT objective across all unsafe prompt categories:
% % \begin{align}
%     d_{\mathrm{OT}}(m) &= \sum_{i=1}^{C}\sum_{n=1}^{N}\mathbf{T}_i(m,n)\,\mathbf{C}_i(m,n), \label{eq:dotm}
% \end{align}
% where $\mathbf{T}_i(m,n)$ is the optimal transport mass from image patch $m$ to the $n$-th textual variant of unsafe category $i$, and $\mathbf{C}_i(m,n)=1-\cos(\mathbf{x}^m,\mathbf{z}_i^n)$ is the semantic transport cost (as defined in Section~\ref{sec:ot_cal}). 
% Intuitively, $d_{\mathrm{OT}}(m)$ is the total OT objective attributed to patch $m$; smaller values indicate that patch $m$ is more closely aligned with unsafe prompts.We then identify unsafe-associated patches using a threshold (or equivalently, by selecting the $K$ smallest scores) and mask them while preserving the rest for reasoning:
% \begin{align}
%     \hat{x}^m &=
%     \begin{cases}
%         0,   & d_{\mathrm{OT}}(m)\le \tau, \\
%         x^m, & \text{otherwise},
%     \end{cases}
% \end{align}
% yielding a sanitized visual input $\hat{x}=\{\hat{x}^m\}_{m=1}^M$ that suppresses unsafe semantics while retaining benign context. Beyond modifying the visual input, we further enhance safety awareness at the textual level by prepending an \emph{interference prefix} (e.g., ``As an AI assistant, ...'') to the user prompt. This lightweight intervention activates the intrinsic safety mechanisms already embedded in MLLMs and steers the generation process toward safe and responsible outputs. Formally, the generation process is written as:
% \begin{equation}
%     y_t \sim \pi_\theta\big(\cdot \mid G(\Phi(\hat{x}), \mathcal{P}, y_{<t})\big), \quad t=1,\dots,T,
% \end{equation}
% where $\hat{x}$ is the masked visual input and $\mathcal{P}$ is the prefix-augmented textual prompt. 


% In summary, masking-guided alignment suppresses unsafe cues at the visual level and reinforces safety at the generation level. 
% This dual mechanism complements the OT-based detection introduced earlier and will be evaluated in the following experiments.


% The OT distance defined in Section~\ref{sec:ot_cal} not only provides a criterion for unsafe-content detection, but also yields patch-level costs that specify which regions are most associated with harmful semantics. Leveraging this property, we compute patch-level OT costs across all unsafe prompt categories to identify regions associated with unsafe semantics. Concretely, we rank the transport costs of all patches and mask those most closely aligned with unsafe prompts, while preserving the rest for reasoning:
% \begin{align}
%      d_{\mathrm{OT}}(m) = \sum_{i=1}^{C}\sum_{n=1}^{N}\mathbf{T}_i(m, n)\mathbf{C}_i(m, n), \quad
%      \hat{x}^m = 
%     \begin{cases}
%         0, & d_{\mathrm{OT}}(m) \leq \tau, \\
%         x^m, & \text{otherwise},
%     \end{cases}
% \end{align}
% Here, $d_{\mathrm{OT}}(m)$ represents the OT cost of patch $m$ with respect to all categorical prompts and $\tau$ is a threshold. Patches with lower $d_{\mathrm{OT}}(m)$ are considered semantically entangled with unsafe prompts and are masked, while those with higher values are preserved. This masking procedure effectively removes regions carrying unsafe semantics, while still retaining sufficient benign context for the model to reason about the task.  


% In summary, masking-guided alignment integrates two complementary mechanisms: patch-level masking eliminates unsafe visual cues at the perception stage, while prefix conditioning reinforces safety alignment during language generation. Together, these mechanisms provide a principled and lightweight safeguard that reduces harmful outputs while preserving task relevance, laying the foundation for the evaluations presented in the next section.

% The OT distance discussed in Section~\ref{sec:ot_cal} not only serves as a quantitative criterion for detecting unsafe content, but also yields patch-level costs that indicate which regions are most associated with harmful semantics. Specifically, for each image patch $m$, we aggregate its transport costs with respect to all unsafe prompt categories:
% \begin{align}
%      d_{\mathrm{OT}}(m) = \sum_{i=1}^{C}\sum_{n=1}^{N}\mathbf{T}_i(m, n)\mathbf{C}_i(m, n), \quad
%      \hat{x}^m = 
%     \begin{cases}
%         0, & d_{\mathrm{OT}}(m) \leq \tau, \\
%         x^m, & \text{otherwise},
%     \end{cases}
% \end{align}
% where $d_{\mathrm{OT}}(m)$ denotes the aggregated OT cost of patch $m$ and $\tau$ is a threshold. Patches with lower $d_{\mathrm{OT}}(m)$ are considered semantically entangled with unsafe prompts and are masked, while patches with higher values are preserved. This masking operation produces a sanitized visual input $\hat{x}$ that suppresses unsafe semantics while retaining benign context.  
% To further strengthen safety awareness during generation, we prepend an \emph{interference prefix} (e.g., ``As an AI assistant, ...'') to the textual prompt. This simple intervention activates the intrinsic safety mechanisms of MLLMs and biases the model toward safe completions. The final generation process is thus formulated as:
% \begin{equation}
%     y_t \sim \pi_\theta\big(\cdot \mid G(\Phi(\hat{x}), \mathcal{P}, y_{<t})\big), \quad t=1,\dots,T,
% \end{equation}
% where $\hat{x}$ is the masked visual input and $\mathcal{P}$ is the textual prompt augmented with the prefix. 
% This masking-guided alignment provides a dual safeguard: patch-level masking eliminates harmful visual cues, while prefix conditioning activates the model’s intrinsic safety capabilities, resulting in responses that are both harmless and contextually relevant.

% where $d_{\mathrm{OT}}(m)$ denotes the aggregated OT cost of patch $m$ with respect to all categorical prompts, and $\tau$ is a threshold. In practice, patches with lower OT cost are regarded as semantically entangled with unsafe prompts and therefore masked, while patches with higher cost are preserved. This masking operation produces a sanitized visual input $\hat{x}$ that suppresses harmful semantics while retaining benign context.
% % To further enhance safety awareness during generation, we prepend an \emph{interference prefix} (e.g., ``As an AI assistant, ...'') to the textual prompt. This encourages the model to maintain a safe response style even when exposed to potentially unsafe content. The final generation process is written as:

% where $\hat{x}$ is the masked visual input and $\mathcal{P}$ is the prefix-augmented textual prompt.  This masking-guided alignment establishes a dual safeguard: (i) patch-level masking removes unsafe visual cues, and (ii) prefix conditioning enhances the model’s safety alignment. Together, these mechanisms ensure that the generated responses remain harmless while preserving contextual relevance.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% This vulnerability is especially challenging
% when benign-looking textual input is combined with visual inputs that implicitly encode malicious intent.
% The attacker aims to induce harmful or policyviolating outputs by submitting image-text queries with malicious intent. Because textual threats are often detected by
% standard safety mechanisms, adversaries typically embed
% malicious intent subtly in the visual input.

% Multimodal Large Language Models (MLLMs) empower the Large Language Models
% (LLMs) with the ability to handle image inputs by integrating a vision encoder, allowing for
% the processing of both textual and visual data.  The input image xv is first encoded by the
% vision encoder V into visual embeddings Zv = V(xv). Then the visual feature is mapped to
% vocabulary embedding space of the LLM via a learnt projector function:

% The projector function may be a simple linear layer (Zhu et al., 2023), an MLP (Liu et al.,
% 2023a), or a re-sampler (Bai et al., 2023; Li et al., 2023b; Dai et al., 2023). The mapped
% image embeddings are concatenated with textual embeddings and provided to the LLM as
% inputs. Given instruction I, textual input query x1:n−1, a pre-trained language model M
% parameterized by θ, and visual tokens Hv, we generate the target answers x
% a by:
% x
% a ∼ M(·|Hv, I, x1:n-1).

% , the vision
% encoder C first converts the image xI into a visual embedding eI . The connector module M then
% projects eI into a continuous sub-space of the textual embedding space, which can serve as input to
% the LLMs. Similar to LLMs, VLMs generate responses by predicting the next token’s distribution in
% an autoregressive manner, continuing to generate tokens until a complete response is produced:


% Multimodal Large Language Models (MLLMs) are autoregressive text generation models that can process multiple
% modalities, such as image [86], video [80], and audio [41],
% in addition to text. In this work, we consider input to MLLM
% in the form of an image and a text prompt. Mathematically,
% we denote a MLLM as a mapping πsafe : I × VN → VM,
% where I represents the image space, and V denotes the vocabulary set. The input to the MLLM πsafe consists of an image
% I ∈ I and a sequence of tokens x := {x1, x2, · · · , xN }
% (referred as prompt), where each token xi ∈ V. Given
% xinput := [I, x], the MLLM πsafe(·|xinput) generates the output sequence y := {y1, y2, · · · , yM}, where yi ∈ V, in a
% token by token fashion.

==> 2026_ICLR/tables/ablation.tex <==
% \renewcommand{\arraystretch}{1.2} 
% \begin{table*}[t]
% \centering
% \begin{minipage}{0.46\linewidth}
% \centering
% \scriptsize 
% \setlength{\tabcolsep}{3pt}
% \caption{Ablation on OT-based adaptive transport vs. cosine similarity for patch selection sensitivity.}
% \label{tab:ablation_a}
% \begin{tabular}{c|ccc}
% \toprule
% \textbf{Model} & \makecell{OT \\ transport} & \makecell{Cosine \\ similarity} & \textbf{Scores} \\
% \midrule
% \multirow{2}{*}{LLaVA-1.5-7B}  
%  & \ding{51} &  &   \\
%  &  & \ding{51} &   \\
% \midrule
% \multirow{2}{*}{LLaVA-1.5-13B}  
%  & \ding{51} &  &   \\
%  &  & \ding{51} &   \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% \hfill
% \begin{minipage}{0.46\linewidth}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \caption{Ablation on framework components.}
% \label{tab:ablation_b}
% \begin{tabular}{c|ccc}
% \toprule
% \textbf{Model} & \makecell{Attention \\ Calibration} & \makecell{Visual \\ Reinforcement} & \textbf{Scores} \\
% \midrule
% \multirow{4}{*}{LLaVA-1.5-7B}  
%  &  &  &   \\
%  & \ding{51} &  &   \\
%  &  & \ding{51} &   \\
%  & \ding{51} & \ding{51} &   \\
% \midrule
% \multirow{4}{*}{LLaVA-1.5-13B}  
%  &  &  &   \\
%  & \ding{51} &  &   \\
%  &  & \ding{51} &   \\
%  & \ding{51} & \ding{51} &   \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% \end{table*}





==> 2026_ICLR/tables/helpful_results.tex <==
% \begin{table}[t]
% \tabstyle{5pt}
% \centering
% \caption{General performance of different methods on LLaVA-1.5-7B and LLaVA-1.5-13B. 
% The first row of each method shows the performance, while the second row shows the difference relative to its VLM backbone. 
% Green indicates improvement, and red indicates a decrease compared to the backbone.}
% \label{tab:helpful}
% \begin{tabular}{c|l|c|cccccc}
% \toprule
% \multirow{3}{*}{Model} & \multirow{3}{*}{Method}  & \multirow{3}{*}{Fine-tuned}  & \multicolumn{4}{c}{\textbf{Comprehensive Benchmark}\hspace{0.2em}{$(\uparrow)$}} & \multicolumn{2}{c}{\textbf{General VQA}\hspace{0.2em}{$(\uparrow)$}} \\
% \cmidrule(lr){4-7} \cmidrule(lr){8-9}
%  &  &  & MME$^{P}$ & MME$^{C}$ & MMB & SQA$^{I}$ & TextVQA & VQAv2 \\
% \midrule
% \multirow{13}{*}{\rotatebox{90}{\textbf{LLaVA-1.5-7B}}}
%  & Original Model &  & 1505.88 & 357.86 & 64.60 & 69.51 & 58.20 & 78.51 \\
% \cmidrule(lr){2-9}
%  & \multirow{2}{*}{+ Posthoc-LoRA} & \multirow{2}{*}{\ding{51}} & 1420.66 & 332.50 & 63.32 & 67.33 & 55.99 & 76.87 \\
%  &  &  & \textcolor{customred}{$\downarrow$85.22} & \textcolor{customred}{$\downarrow$25.36} & \textcolor{customred}{$\downarrow$1.28} & \textcolor{customred}{$\downarrow$2.18} & \textcolor{customred}{$\downarrow$2.21} & \textcolor{customred}{$\downarrow$1.64} \\
% \cmidrule(lr){2-9}
%  & \multirow{2}{*}{+ Mixed-LoRA} & \multirow{2}{*}{\ding{51}} & 1483.00 & 267.14 & \textbf{68.04} & 68.42 & 57.88 & \textbf{79.18} \\
%  &  &  & \textcolor{customred}{$\downarrow$22.88} & \textcolor{customred}{$\downarrow$90.72} & \textcolor{customgreen}{$\uparrow$3.44} & \textcolor{customred}{$\downarrow$1.09} & \textcolor{customred}{$\downarrow$0.32} & \textcolor{customgreen}{$\uparrow$0.67} \\
% \cmidrule(lr){2-9}
%  & \multirow{2}{*}{+ ECSO} & \multirow{2}{*}{\ding{55}} & 1495.88 & \textbf{360.00} & 63.83 & 69.36 & 58.15 & 78.39 \\
%  &  &  & \textcolor{customred}{$\downarrow$10.00} & \textcolor{customgreen}{$\uparrow$2.14} & \textcolor{customred}{$\downarrow$0.77} & \textcolor{customred}{$\downarrow$0.15} & \textcolor{customred}{$\downarrow$0.05} & \textcolor{customred}{$\downarrow$0.12} \\
% \cmidrule(lr){2-9}
%  & \multirow{2}{*}{+ ETA} & \multirow{2}{*}{\ding{55}} & \textbf{1506.13} & 357.86 & 64.69 & \textbf{69.51} & \textbf{58.15} & 78.51 \\
%  &  &  & \textcolor{customgreen}{$\uparrow$0.25} & \textcolor{customgreen}{$\uparrow$0.00} & \textcolor{customgreen}{$\uparrow$0.09} & \textcolor{customgreen}{$\uparrow$0.00} & \textcolor{customred}{$\downarrow$0.05} & \textcolor{customgreen}{$\uparrow$0.00} \\
% \cmidrule(lr){2-9}
%  & \multirow{2}{*}{+ $\ours$} & \multirow{2}{*}{\ding{55}} & \textbf{1506.13} & 357.86 & 64.69 & \textbf{69.51} & \textbf{58.15} & 78.51 \\
%  &  &  & \textcolor{customgreen}{$\uparrow$0.25} & \textcolor{customgreen}{$\uparrow$0.00} & \textcolor{customgreen}{$\uparrow$0.09} & \textcolor{customgreen}{$\uparrow$0.00} & \textcolor{customred}{$\downarrow$0.05} & \textcolor{customgreen}{$\uparrow$0.00} \\
%  \midrule
% \multirow{13}{*}{\rotatebox{90}{\textbf{\textcolor{black}{LLaVA-1.5-13B}}}} 
%  & Original Model &  & 1528.77 & 296.07 & 68.38 & 72.78 & 61.21 & 79.99 \\
% \cmidrule(lr){2-9}
%  & \multirow{2}{*}{+ Posthoc-Lora} & \multirow{2}{*}{\ding{51}} & 1510.13 & \textbf{318.57} & 66.58 & 71.29 & 59.15 & 78.50 \\
%  & & & \textcolor{customred}{$\downarrow$18.64} & \textcolor{customgreen}{$\uparrow$22.50} & \textcolor{customred}{$\downarrow$1.80} & \textcolor{customred}{$\downarrow$1.49} & \textcolor{customred}{$\downarrow$2.06} & \textcolor{customred}{$\downarrow$1.49} \\
% \cmidrule(lr){2-9}
%  & \multirow{2}{*}{+ Mixed-Lora} & \multirow{2}{*}{\ding{51}} & \textbf{1579.89} & 258.21 & 68.21 & 71.94 & 60.35 & \textbf{80.13} \\
%  & & & \textcolor{customgreen}{$\uparrow$51.12} & \textcolor{customred}{$\downarrow$37.86} & \textcolor{customred}{$\downarrow$0.17} & \textcolor{customred}{$\downarrow$0.84} & \textcolor{customred}{$\downarrow$0.86} & \textcolor{customgreen}{$\uparrow$0.14} \\
% \cmidrule(lr){2-9}
%  & \multirow{2}{*}{+ ECSO} & \multirow{2}{*}{\ding{55}} & 1523.76 & 296.07 & 66.49 & 72.83 & 61.04 & 79.89 \\
%  & & & \textcolor{customred}{$\downarrow$5.01} & \textcolor{customgreen}{$\uparrow$0.00} & \textcolor{customred}{$\downarrow$1.89} & \textcolor{customgreen}{$\uparrow$0.05} & \textcolor{customred}{$\downarrow$0.17} & \textcolor{customred}{$\downarrow$0.10} \\
% \cmidrule(lr){2-9}
%  & \multirow{2}{*}{+ ETA} & \multirow{2}{*}{\ding{55}} & 1531.19 & 296.07 & \textbf{68.38} & \textbf{72.83} & \textbf{61.09} & 79.99 \\
%  & & & \textcolor{customgreen}{$\uparrow$2.42} & \textcolor{customgreen}{$\uparrow$0.00} & \textcolor{customgreen}{$\uparrow$0.00} & \textcolor{customgreen}{$\uparrow$0.05} & \textcolor{customred}{$\downarrow$0.12} & \textcolor{customgreen}{$\uparrow$0.00} \\
% \cmidrule(lr){2-9}
%  & \multirow{2}{*}{+ $\ours$} & \multirow{2}{*}{\ding{55}} & 1531.19 & 296.07 & \textbf{68.38} & \textbf{72.83} & \textbf{61.09} & 79.99 \\
%  & & & \textcolor{customgreen}{$\uparrow$2.42} & \textcolor{customgreen}{$\uparrow$0.00} & \textcolor{customgreen}{$\uparrow$0.00} & \textcolor{customgreen}{$\uparrow$0.05} & \textcolor{customred}{$\downarrow$0.12} & \textcolor{customgreen}{$\uparrow$0.00} \\
% \bottomrule
% \end{tabular}\vspace{-5pt}
% \end{table}

\begin{table}[t]
\tabstyle{5.5pt}
\centering
\caption{General performance of different methods.}
\label{tab:helpful}
\begin{tabular}{c|l|c|cccccc}
\toprule
\multirow{3}{*}{Model} & \multirow{3}{*}{Method}  & \multirow{3}{*}{Fine-tuned}  & \multicolumn{4}{c}{\textbf{Comprehensive Benchmark}\hspace{0.2em}{$(\uparrow)$}} & \multicolumn{2}{c}{\textbf{General VQA}\hspace{0.2em}{($\uparrow$)}} \\
\cmidrule(lr){4-7} \cmidrule(lr){8-9}
 &  &  & MME$^{P}$ & MME$^{C}$ & MMB & SQA$^{I}$ & TextVQA & VQAv2 \\
\midrule
\multirow{7}{*}{\rotatebox{90}{\textbf{LLaVA-1.5-7B}}}
 &  Vanilla MLLM &  & 1505.88 & 357.86 & 64.60 & 69.51 & 58.20 & 78.51 \\
\cmidrule(lr){2-9}
 & {+ Posthoc-LoRA} & {\ding{51}} & 1420.66 & 332.50 & 63.32 & 67.33 & 55.99 & 76.87 \\
 & {+ Mixed-LoRA} & {\ding{51}} & 1483.00 & 267.14 & \textbf{68.04} & 68.42 & 57.88 & {79.18} \\
 & {+ ECSO} & {\ding{55}} & 1495.88 & \textbf{360.00} & 63.83 & 69.36 & 58.15 & 78.39 \\
 & {+ ETA} & {\ding{55}} & {1506.13} & 357.86 & 64.69 & {69.51} & {58.15} & 78.51 \\
 & {+ $\ours$} & {\ding{55}} & \textbf{1508.29} & \textbf{363.65} & 65.68 & \textbf{70.23} & \textbf{58.95} & \textbf{79.21} \\
 \midrule
\multirow{7}{*}{\rotatebox{90}{\textbf{\textcolor{black}{LLaVA-1.5-13B}}}} 
 & Vanilla MLLM &  & 1528.77 & 296.07 & 68.38 & 72.78 & 61.21 & 79.99 \\
\cmidrule(lr){2-9}
 & {+ Posthoc-Lora} & {\ding{51}} & 1510.13 & \textbf{318.57} & 66.58 & 71.29 & 59.15 & 78.50 \\
 & {+ Mixed-Lora} & {\ding{51}} & \textbf{1579.89} & 258.21 & 68.21 & 71.94 & 60.35 & \textbf{80.13} \\
 & {+ ECSO} & {\ding{55}} & 1523.76 & 296.07 & 66.49 & 72.83 & 61.04 & 79.89 \\
 & {+ ETA} & {\ding{55}} & 1531.19 & 296.07 & {68.38} & {72.83} & {61.09} & 79.99 \\
 & {+ $\ours$} & {\ding{55}} & 1533.28 & 296.07 & \textbf{69.52} & \textbf{73.693} & \textbf{62.13} & \textbf{80.25} \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[t]
\tabstyle{10pt}
\centering
\caption{Helpfulness evaluation on the SPA-VL Help.}\label{tab:ai_eval}
% \vspace{-5pt}
% \fontsize{9pt}{11pt}\selectfont 
\begin{tabular}{l| cc| c }
\toprule
\textbf{Model} & \multicolumn{2}{c|}{\textbf{Comparison Methods}} & \textbf{Win-Tie (\%) $\uparrow$} \\
% \cmidrule(lr){2-3}
               % & \textbf{ETA vs} & \textbf{Method} & \\ 
\midrule
\multirow{5}{*}{LLaVA-1.5-7B}  
   & \multirow{5}{*}{$\ours$ \quad v.s.} & Vanilla VLM   & 93.6 \\ 
   &                      & Posthoc-LoRA  & 53.2 \\ 
   &                      & Mixed-LoRA    & 55.7 \\ 
   &                      & ECSO          & 85.3 \\ 
   &                      & ETA          & 79.8 \\ 
\midrule
\multirow{5}{*}{LLaVA-1.5-13B}  
   & \multirow{5}{*}{$\ours$ \quad v.s.} & Vanilla VLM   & 90.2 \\ 
   &                      & Posthoc-LoRA  & 52.8 \\ 
   &                      & Mixed-LoRA    & 53.5 \\ 
   &                      & ECSO          & 83.8 \\ 
   &                      & ETA          & 78.6 \\ 
\bottomrule
\end{tabular}
\end{table}










% \begin{table}[t]
% \tabstyle{5pt}
% \centering
% \caption{General performance of different methods on LLaVA-1.5-7B. The first row of each method shows the performance, while the second row shows the difference relative to its VLM backbone. \textcolor{customgreen}{Green} indicates improvement, and \textcolor{customred}{red} indicates a decrease compared to the VLM backbone. Our method outperforms other finetune-based and inference-time baselines.}\label{tab:helpful}
% % \vspace{-5pt}
% % \fontsize{9pt}{10pt}\selectfont
% \begin{tabular}{l|c|cccccc}
% % {l@{\hskip 1.5mm}|@{\hskip 1.5mm}c@{\hskip 1.5mm}|ccccc@{\hskip 2mm}c}
% \toprule
%  &  & \multicolumn{4}{c}{\textbf{Comprehensive Benchmark}} & \multicolumn{2}{c}{\textbf{General VQA}} \\
% \cmidrule(lr){3-6} \cmidrule(lr){7-8}
% Method & Fine-tuned & MME$^{P}$ & MME$^{C}$ & MMB & SQA$^{I}$ & TextVQA & VQAv2 \\
% \midrule
% LLaVA-1.5-7B &  & 1505.88 & 357.86 & 64.60 & 69.51 & 58.20 & 78.51 \\
% \midrule
% \multirow{2}{*}{+ Posthoc-LoRA} & \multirow{2}{*}{\ding{51}} & 1420.66 & 332.50 & 63.32 & 67.33 & 55.99 & 76.87 \\
%  &  & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}85.22} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}25.36} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}1.28} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}2.18} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}2.21} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}1.64} \\
% \midrule
% \multirow{2}{*}{+ Mixed-LoRA} & \multirow{2}{*}{\ding{51}} & 1483.00 & 267.14 & \textbf{68.04} & 68.42 & 57.88 & \textbf{79.18} \\
% &  & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}22.88} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}90.72} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}3.44}} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}1.09} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}0.32} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}0.67}} \\
% \midrule
% \multirow{2}{*}{+ ECSO} & \multirow{2}{*}{\ding{55}} & 1495.88 & \textbf{360.00} & 63.83 & 69.36 & 58.15 & 78.39 \\
% &  & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}10.00} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}2.14}} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}0.77} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}0.15} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}0.05} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}0.12} \\
% \midrule
% \multirow{2}{*}{+ ETA} & \multirow{2}{*}{\ding{55}} & \textbf{1506.13} & 357.86 & 64.69 & \textbf{69.51} & \textbf{58.15} & 78.51 \\
%  &  & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}0.25}} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.00} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.09} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}0.00}} & \textcolor{customred}{\textbf{\raisebox{0.4ex}{$\downarrow$}0.05}} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.00} \\
%  \midrule
%  \multirow{2}{*}{+ $\ours$} & \multirow{2}{*}{\ding{55}} & \textbf{1506.13} & 357.86 & 64.69 & \textbf{69.51} & \textbf{58.15} & 78.51 \\
%  &  & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}0.25}} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.00} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.09} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}0.00}} & \textcolor{customred}{\textbf{\raisebox{0.4ex}{$\downarrow$}0.05}} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.00} \\
% \bottomrule
% \end{tabular}\vspace{-5pt}
% \end{table}




% \begin{table}[t]
% \tabstyle{5pt}
% \centering
% \caption{General performance of different methods on LLaVA-1.5-13B.}\label{tab:helpful13b}
% % \fontsize{9pt}{11pt}\selectfont
% \begin{tabular}{l|c|cccccc}
% % {l@{\hskip 1.5mm}|@{\hskip 1.5mm}c@{\hskip 1.5mm}|ccccc@{\hskip 3mm}c}
% \toprule
% \multirow{2}{*}{Method} & \multirow{2}{*}{Fine-tuned} & \multicolumn{4}{c}{\textbf{Comprehensive Benchmark}} & \multicolumn{2}{c}{\textbf{General VQA}} \\
% \cmidrule(lr){3-6} \cmidrule(lr){7-8}
%  &  & MME$^{P}$ & MME$^{C}$ & MMB & SQA$^{I}$ & TextVQA & VQAv2 \\
% \midrule
% LLaVA-1.5-13B & & 1528.77 & 296.07 & 68.38 & 72.78 & 61.21 & 79.99 \\
% \midrule
% \multirow{2}{*}{+ VLGuard-Posthoc-Lora} & \multirow{2}{*}{\ding{51}} & 1510.13 & \textbf{318.57} & 66.58 & 71.29 & $59.15$ & 78.50 \\
%  & & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}18.64} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}22.50}} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}1.80} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}1.49} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}2.06} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}1.49} \\
% \midrule
% \multirow{2}{*}{+ VLGuard-Mixed-Lora} & \multirow{2}{*}{\ding{51}} & \textbf{1579.89} & 258.21 & 68.21 & 71.94 & 60.35 & \textbf{80.13} \\
% & & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}51.12}} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}37.86} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}0.17} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}0.84} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}0.86} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}0.14}} \\
% \midrule
% \multirow{2}{*}{+ ECSO} & \multirow{2}{*}{\ding{55}} & 1523.76 & 296.07 & 66.49 & 72.83 & 61.04 & 79.89 \\
% & & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}5.01} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.00} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}1.89} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.05} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}0.17} & \textcolor{customred}{\raisebox{0.4ex}{$\downarrow$}0.10} \\
% \midrule
% \multirow{2}{*}{+ ETA} & \multirow{2}{*}{\ding{55}} & 1531.19 & 296.07 & \textbf{68.38} & \textbf{72.83} & \textbf{61.09} & 79.99 \\
% & & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}2.42} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.00} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}0.00}} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}0.05}} & \textcolor{customred}{\textbf{\raisebox{0.4ex}{$\downarrow$}0.12}} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.00} \\
% \midrule
% \multirow{2}{*}{+ $\ours$} & \multirow{2}{*}{\ding{55}} & 1531.19 & 296.07 & \textbf{68.38} & \textbf{72.83} & \textbf{61.09} & 79.99 \\
% & & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}2.42} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.00} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}0.00}} & \textcolor{customgreen}{\textbf{\raisebox{0.4ex}{$\uparrow$}0.05}} & \textcolor{customred}{\textbf{\raisebox{0.4ex}{$\downarrow$}0.12}} & \textcolor{customgreen}{\raisebox{0.4ex}{$\uparrow$}0.00} \\
% \bottomrule
% \end{tabular}
% \end{table}




==> 2026_ICLR/tables/model_mask_case.tex <==
\begin{figure}[!t]
\centering
\begin{minipage}{0.45\textwidth}
    \centering
    \begin{subfigure}[b]{1\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{2026_ICLR/figures/clip_model_ablation.pdf}
    \end{subfigure}
    \caption{Comparison of SPA-VL harm rates and TextVQA performance across different CLIP backbones.}
    \label{fig:clip_backbone}
\end{minipage}
\quad
\begin{minipage}{0.45\textwidth}
    \centering
    \begin{subfigure}[b]{1\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{2026_ICLR/figures/case_study.pdf}
    \end{subfigure}
    \caption{Examples of mask-guided alignment. Unsafe regions in the original image are automatically detected and masked.}
    \label{fig:mask_case}
\end{minipage}
% \vspace{-0.5cm}
\end{figure}


==> 2026_ICLR/tables/rebuttal_epsion_reg.tex <==
\begin{table}[!ht]
\centering
\tabstyle{5pt}
{\color{RoyalBlue}
\caption{\textblue{Results under different regularization strengths $\epsilon$.}}
\label{tab:adv_eps}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{$\epsilon = 0.01$}
& \multicolumn{2}{c}{$\epsilon = 0.05$}
& \multicolumn{2}{c}{$\epsilon = 0.1$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\textbf{Model} &
$\text{CHAIR}_S\downarrow$ & {BLEU}$\uparrow$ &
$\text{CHAIR}_S\downarrow$ & {BLEU}$\uparrow$ &
$\text{CHAIR}_S\downarrow$ & {BLEU}$\uparrow$ \\
\midrule
LLaVA-1.5 & 22.0 & 14.5 & 22.0 & 14.5 & 22.0 & 14.5  \\
\textbf{AIR} & 18.5 & 14.5 & 18.3 & 14.6 & 18.4 & 14.4 \\
\bottomrule
\end{tabular}}
\end{table}


==> 2026_ICLR/tables/safety_ASR_reuslts.tex <==
\begin{table}[t]
\tabstyle{4pt}
\centering
\caption{ASR performance across multiple safety benchmarks.}\label{tab:asr}
% \fontsize{9pt}{11pt}\selectfont
\begin{tabular}{l|ccccc}
% {l@{\hskip 1.2mm}|ccc@{\hskip 1.5mm}cc}
\toprule
\multirow{2.5}{*}{Method}& \textbf{SPA-VL} & \textbf{MM-SafetyBench} & \multicolumn{2}{c}{\textbf{FigStep}} & \textbf{Adv. Image+Text} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-6}
 & Harm\hspace{0.2em}$\downarrow$ & SD+TYPO\hspace{0.2em}$\downarrow$ & Vanilla\hspace{0.2em}$\downarrow$ & Suffix\hspace{0.2em}$\downarrow$ & Unconstrained\hspace{0.2em}$\downarrow$ \\
\midrule
LLaVA-1.5-7B & 72.45 & 84.46 & 86.40 & 85.80 & 85.00 \\
+ ECSO & 53.96 & 72.44 & 79.29 & 82.20 & 67.50  \\
+ ETA & {38.87} & {53.39} & {32.40} & {25.00} & {17.50} \\
+ $\ours$ & \textbf{32.71} & \textbf{45.52} & \textbf{25.40} & \textbf{20.00} & \textbf{13.00} \\
\midrule
LLaVA-1.5-13B & 66.79 & 87.98 & 90.20 & 87.40 & 80.00 \\
+ ECSO & 47.92 & 68.57 & 53.80 & 85.60 & 67.50 \\
+ ETA & {39.62} & {46.19} & {28.80} & {6.80} & {12.50} \\
+ \ours & \textbf{33.37} & \textbf{39.29} & \textbf{22.50} & \textbf{3.00} & \textbf{8.00} \\
\midrule
InternVL-Chat-1.0-7B & 72.08 & 85.77 & 85.80 & 85.20 & 85.00 \\
+ ECSO & 56.23 & 75.06 & 86.00 & 84.00 & 70.00 \\
+ ETA & {43.40} & {56.25} & {42.40} & {31.80} & {20.00} \\
+ $\ours$ & \textbf{35.650} & \textbf{48.37} & \textbf{35.50} & \textbf{26.50} & \textbf{14.00} \\
\midrule
InternLM-XComposer-2.5-7B & 61.51 & 74.29 & 57.80 & 86.60 & 17.50 \\
+ ECSO & 55.09 & 73.10 & 59.20 & 86.80 & 15.00 \\
+ ETA & {45.28} & {60.65} & {38.00} & {45.00} & {15.00}\\
+ $\ours$ & \textbf{37.58} & \textbf{52.65} & \textbf{31.80} & \textbf{36.00} & \textbf{10.50} \\
\bottomrule
\end{tabular}
\end{table}












% \begin{table}[t]
% \tabstyle{9pt}
% \centering
% \caption{Performance on text only safety benchmark.}\label{tab:advbench}
% % \fontsize{9pt}{11pt}\selectfont
% \begin{tabular}{l|cccc}
% \toprule
% \multirow{3}{*}{Method}& \multicolumn{2}{c}{\textbf{AdvBench (USR)}} & \multicolumn{2}{c}{\textbf{AdvBench (ASR)}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
%  & Vanilla\hspace{0.2em}$\downarrow$ & Suffix\hspace{0.2em}$\downarrow$  & Vanilla\hspace{0.2em}$\downarrow$ & Suffix\hspace{0.2em}$\downarrow$  \\
% \midrule
% LLaVA-1.5-7B & 10.77 & 98.85 & 4.23 & 41.73 \\
% + ECSO & 3.08 & 90.19 & 0.58 & 41.73 \\
% + ETA & \textbf{3.08} & \textbf{2.31} & \textbf{0.38} & \textbf{0.77} \\
% + $\ours$ & \textbf{3.08} & \textbf{2.31} & \textbf{0.38} & \textbf{0.77} \\
% \midrule
% LLaVA-1.5-13B & 1.92 & 96.92 & 1.73 & 34.43 \\
% + ECSO & 2.12 & 86.35 & 0.96 & 43.27 \\
% + ETA & \textbf{0.77} & \textbf{1.92} & \textbf{0.58} & \textbf{0.77} \\
% + $\ours$ & \textbf{3.08} & \textbf{2.31} & \textbf{0.38} & \textbf{0.77} \\
% \midrule
% InternVL-Chat-1.0-7B & 11.15 & 97.12 & 4.81 & 41.54 \\
% + ECSO & \textbf{2.89} & 90.58 & 1.35 & 0.38 \\
% + ETA & 4.04 & \textbf{1.35} & \textbf{0.58} & \textbf{0.38} \\
% + $\ours$ & \textbf{3.08} & \textbf{2.31} & \textbf{0.38} & \textbf{0.77} \\
% \midrule
% InternLM-XComposer-2.5-7B & 0.00 & 37.31 & 0.00 & 21.92 \\
% + ECSO & 0.00 & 10.96 & 0.19 & 7.12 \\
% + ETA & \textbf{0.00} & \textbf{5.00} & \textbf{0.00} & 
% \textbf{4.23} \\
% + $\ours$ & \textbf{3.08} & \textbf{2.31} & \textbf{0.38} & \textbf{0.77} \\
% \bottomrule
% \end{tabular}
% \end{table}


==> 2026_ICLR/tables/safety_USR_results.tex <==
\begin{table}[t]
\tabstyle{5pt}
\centering
\caption{USR evaluation results across multiple safety benchmarks. }\label{tab:usr}
% \vspace{-5pt}
% \fontsize{9pt}{10pt}\selectfont
\begin{tabular}{l|ccccc}
\toprule
\multirow{2.5}{*}{Method} & \textbf\textbf{SPA-VL} & \textbf\textbf{MM-SafetyBench} & \multicolumn{2}{c}{\textbf\textbf{FigStep}} & \textbf\textbf{Adv. Image+Text} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-6}
 & Harm\hspace{0.2em}$\downarrow$ & SD+TYPO\hspace{0.2em}$\downarrow$ & Vanilla\hspace{0.2em}$\downarrow$ & Suffix\hspace{0.2em}$\downarrow$ & Unconstrained\hspace{0.2em}$\downarrow$ \\
\midrule
LLaVA-1.5-7B & 46.04 & 40.46 & 58.60 & 62.00 & 97.50 \\
+ ECSO & 23.40 & 15.89 & 37.40 & 59.00 & 95.00 \\
+ ETA & {16.98} & {15.83} & {7.80} & {22.60} & {22.50} \\
+ $\ours$ &\textbf{10.31} &\textbf{9.65} &\textbf{3.40} &\textbf{15.30} &\textbf{15.00} \\
\midrule
LLaVA-1.5-13B & 40.75 & 41.01 & 61.60 & 66.40 & 100.00 \\
+ ECSO & 15.47 & 13.81 & \textbf{15.00} & 37.20 & 95.00 \\
+ ETA & {15.09} & {11.67} & 22.60 & {20.80} & {12.50} \\
+ $\ours$ &\textbf{11.36} &\textbf{9.81} &\textbf{14.29} &\textbf{16.30} &\textbf{6.50} \\
\midrule
InternVL-Chat-1.0-7B & 46.79 & 37.20 & 47.40 & 52.80 & 97.50 \\
+ ECSO & 28.68 & 15.54 & 41.20 & 49.40 & 95.00 \\
+ ETA & {16.98} & {13.81} & {17.40} & {10.80} & {25.00} \\
+ $\ours$ &\textbf{12.58} &\textbf{10.63} &\textbf{12.50} &\textbf{8.60} &\textbf{18.00} \\
\midrule
InternLM-XComposer-2.5-7B & 27.55 & 21.79 & 22.60 & 50.80 & 7.50 \\
+ ECSO & 19.62 & 14.94 & 16.60 & 42.40 & 5.00 \\
+ ETA & {13.96} & {7.32} & {6.00} & {7.20} & {5.00} \\
+ $\ours$ &\textbf{8.26} &\textbf{5.62} &\textbf{4.50} &\textbf{5.30} &\textbf{3.50} \\
\midrule
LLaVA-NeXT-8B & 23.02 & 30.18 & 49.40 & 63.40 & 62.50 \\
% + ECSO & 23.40 & 15.89 & 37.40 & 59.00 & 95.00 \\
+ ECSO & 17.69 &  25.86 & 37.50 & 48.20 & 59.50\\
+ ETA & {11.32} & {10.48} & {20.60} & {19.60} & {17.50} \\
+ $\ours$ & \textbf{8.92} & \textbf{7.25} & \textbf{17.60} & \textbf{15.80} & \textbf{14.50} \\
\midrule
LLaVA-OneVision-7B-Chat & 15.85 & 29.76 & 45.20 & 40.40 & 70.00 \\ 
+ ECSO & 13.56 & 25.34 & 38.40 & 33.60 & 53.20 \\
+ ETA & {6.79} & {10.60} & {16.80} & {19.40} & {20.00} \\
+ $\ours$ & \textbf{5.21} & \textbf{6.48} & \textbf{11.20} & \textbf{13.50} & \textbf{15.00} \\
\midrule
Llama3.2-11B-Vision-Instruct & 7.17 & 19.17 & 41.60 & 44.00 & 15.00 \\
+ ECSO & 6.58 & 16.78 & 35.20 & 33.50 &13.50 \\
+ ETA & {2.64} & {3.99} & {8.20} & {3.20} & {7.50} \\
+ $\ours$ & \textbf{1.25} & \textbf{2.28} & \textbf{3.50} & \textbf{3.00} &\textbf{3.50} \\
\bottomrule
\end{tabular}
% \vspace{-10pt}
\end{table}


%SPA-VL 265条数据
%Attack 40条数据
%MM_SafetyBench_eta_results 1680条数据


